Unbalanced Optimal Transport: Dynamic and Kantorovich Formulation

This article presents a new class of distances between arbitrary nonnegative Radon measures inspired by optimal transport. These distances are defined by two equivalent alternative formulations: (i) a dynamic formulation defining the distance as a geodesic distance over the space of measures (ii) a static "Kantorovich" formulation where the distance is the minimum of an optimization problem over pairs of couplings describing the transfer (transport, creation and destruction) of mass between two measures. Both formulations are convex optimization problems, and the ability to switch from one to the other depending on the targeted application is a crucial property of our models. Of particular interest is the Wasserstein-Fisher-Rao metric recently introduced independently by Chizat et al. and Kondratyev et al. Defined initially through a dynamic formulation, it belongs to this class of metrics and hence automatically benefits from a static Kantorovich formulation.

==> Submission Final JFA/Abstract.tex <==
% !TEX root = ../DynamicToStatic.tex

\begin{abstract}
This article presents a new class of distances between arbitrary nonnegative Radon measures inspired by optimal transport. These distances are defined by two equivalent alternative formulations: (i) a \emph{dynamic} formulation defining the distance as a geodesic distance over the space of measures (ii) a static ``Kantorovich'' formulation where the distance is the minimum of an optimization problem over pairs of couplings describing the transfer (transport, creation and destruction) of mass between two measures. Both formulations are convex optimization problems, and the ability to switch from one to the other depending on the targeted application is a crucial property of our models. 
%
Of particular interest is the Wasserstein-Fisher-Rao metric recently introduced independently by~\cite{ChizatOTFR2015,new2015kondratyev}. Defined initially through a dynamic formulation, it belongs to this class of metrics and hence automatically benefits from a static Kantorovich formulation. %Switching from the initial Eulerian expression of this metric to a Lagrangian point of view provides the generalization of Otto's Riemannian submersion to this new setting, where the group of diffeomorphisms is replaced by a semi-direct product of groups.
%
%This Riemannian submersion enables a formal computation of the sectional curvature of the space of densities and the formulation of an equivalent Monge problem. 
% Then, we develop a new Kantorovich formulation and prove a correspondence result between the dynamical formulations and Kantorovich formulations. As an application, we obtain the Kantorovich formulation of the model introduced in~\cite{ChizatOTFR2015} and we develop a Gamma-convergence result of the model to  standard optimal transport.
\end{abstract}


==> Submission Final JFA/Conclusion.tex <==
% !TEX root = ../DynamicToStatic.tex

\section*{Conclusion and Perspectives}

In this paper, we presented a unified treatment of unbalanced optimal transport that allows for both static and dynamic formulations. Our key findings are (i) a new class of dynamic unbalanced optimal transport problems, (ii) a new class of static optimal transport formulations involving semi-couplings, (iii) an equivalence between these static formulations and a class of dynamic formulations. 
%Each of these contributions is of independent interest, but the synergy between the dynamic and the static problems allows to get a clear picture of the unbalanced transportation problem. Beside these theoretical advances, w
We believe that a key aspect of this work is that the proposed static formulation opens the door to a new class of numerical solvers for unbalanced optimal transport. These solvers should leverage the specific structure of the cost $c$ considered for each application, a striking example being the $\WF$ cost~\eqref{eq:GeneralizedCost:OTFR}.

% we studied the geometry of a generalized optimal transport and we established a correspondence between dynamic formulations of these models and a new Kantorovich formulation. This is a key improvement for numerical efficiency.

%%%%
\section*{Acknowledgements}

The work of Bernhard Schmitzer has been supported by the Fondation Sciences Math\'ematiques de Paris. 
%
The work of Gabriel Peyr\'e has been supported by the European Research Council (ERC project SIGMA-Vision). 
%
The work of Fran\c{c}ois-Xavier Vialard has been supported by the CNRS (D\'efi Imag'in de la Mission pour l'Interdisciplinarit\'e, project CAVALIERI).
%
\\
We would like to thank Yann Brenier for stimulating discussions.% as well as Peter Michor, in particular for several important references.



==> Submission Final JFA/Dynamic.tex <==
% !TEX root = ../DynamicToStatic.TEX

%%%%%%%%%%%%%%%%%%%%%%%%%
% DYNAMIC
%%%%%%%%%%%%%%%%%%%%%%%%%

\section{A Family of Dynamic Problems}\label{sec:dynamic}
In this section, we describe a first approach to unbalanced optimal transport, which generalizes~\eqref{eq:WFInformal} and is inspired by the \emph{dynamic} formulation of classical optimal transport. 
%In this section we establish that a certain class of convex, positively homogeneous, optimization problems over the solutions of the continuity equation with source (informally introduced in \ref{eq:ContinuityEqInformal}) --- the dynamic problems --- admits unbalanced Kantorovich formulations that we introduced in Sect.\ \ref{sec : general static problem} --- the static problems.
%We prove an equivalence result between static and dynamic models for a large class of dynamic models.
%It is however not the aim of this manuscript to exhaust the full class of dynamic problems that allow for a static reformulation.
%As a direct application of this result, we obtain the equivalence for $\WF$ in section~\ref{sec:Examples}.
%%\label{sec : proof static}
%
Dynamic formulations of unbalanced transport models correspond intuitively to the computation of geodesic distances according to a function 
measuring the infinitesimal effort needed for ``acting'' on a mass $\rho$ at position $x$ according to the speed $v$ and rate of growth $g$ (cf.~\eqref{eq:DynamicInformal}). In this section, $\Omega$ is the closure of an open, connected, bounded subset of $\R^d$ with Lipschitz boundary.
%This should be contrasted with the static formulation~\eqref{eq: static problem} that depends on a cost function $c(x_0,m_0,x_1,m_1)$ between pairs of positions and masses.
%\todo{Len: I modified the previous paragraph; to me $f$ only appears after a change of variables}

\subsection{Continuity equation}
The continuity equation, informally introduced in \eqref{eq:ContinuityEqInformal}, is a key concept for the dynamic formulations of this article. It enforces a local mass preservation constraint for a density $\rho$, a flow field $v$ and a growth rate field $g$.
We now give a rigorous definition in terms of measures $(\rho,\omega,\zeta)$ where $\omega$ can informally be interpreted as the momentum $\rho \cdot v$ of the flow field and $\zeta$ corresponds to $\rho \cdot g$. As opposed to what is standard in the literature, we do not require a priori $\omega$ and $\zeta$ to have a density with respect to $\rho$ : this allows to deal with a wider class of action functionals.
%
\begin{definition}[Continuity equation with source]
\label{def:continuity equation}
For $(a,b)\in \R^2$ and a compact domain $\Omega \subset \R^d$, denote by $\mathcal{CE}_a^b(\rho_0,\rho_1)$ the affine subset of $\mathcal{M}([a,b]\times \Omega)\times \mathcal{M}([a,b]\times \Omega)^d \times \mathcal{M}([a,b]\times \Omega)$ of triplets of measures $\mu=(\rho,\omega,\zeta)$ satisfying the continuity equation 
\[
\partial_t \rho + \nabla \cdot \omega = \zeta
\]
 in the distributional sense, interpolating between $\rho_0$ and $\rho_1$ and satisfying homogeneous Neumann boundary conditions. More precisely we require
\begin{equation}
\label{eq:continuity weak}
\int_a^b \int_{\Omega} \partial_t \varphi \ \d\rho + \int_a^b \int_{\Omega} \nabla \varphi \cdot \d\omega + \int_a^b \int_{\Omega} \varphi \ \d\zeta = \int_{\Omega} \varphi(b,\cdot)\d\rho_1 - \int_{\Omega} \varphi(a,\cdot)\d\rho_0
\end{equation}
for all $\varphi \in C^1([a,b]\times \Omega)$.
\end{definition}
%
Below we collect two simple facts on this equation which will turn out useful. Their proof only involves elementary operations that we do not reproduce here for conciseness. The notation $B^d(0,r)$ denotes the open ball of radius $r$ in $\R^d$ centered at the origin.
\begin{proposition}
\label{prop:results on continuity equation}
\hfill
\begin{description}
%\item[Glueing] Let $(a,b,c) \in \R^3$ satisfying $a<b<c$, $(\rho_a,\rho_b,\rho_c) \in \mathcal{M}_+(\Omega)^3$, $\mu_A \in \mathcal{CE}_a^b(\rho_a,\rho_b)$ and $\mu_B \in \mathcal{CE}_b^c(\rho_b,\rho_c)$. Then the measure $\mu$ defined as $\mu_A$ for $t\in [a,b[$ and $\mu_B$ for $t\in [b,c]$ belongs to $\mathcal{CE}_a^c(\rho_a,\rho_c)$.
%\item[Extension.] Let $(a,b,c) \in \R^3$ satisfying $a<b<c$, $(\rho_a,\rho_b) \in \mathcal{M}_+(\Omega)^2$ and $\mu \in \mathcal{CE}_a^b(\rho_a,\rho_b)$. Then the measure $\tilde{\mu}$ obtained by extending $\mu$ as $(\rho_b , 0, 0)\otimes \d t$ on $]b,c]\times \Omega$ belongs to $\mathcal{CE}_a^c(\rho_a,\rho_b)$.
%
\item[Smoothing.] Let $\veps>0$, let $r^x_{\veps}$, $r^t_\veps$ mollifiers supported on the open balls $B^d(0,\frac{\veps}{2})$ and $B^1(0,\frac{\veps}{2})$ respectively and $r_{\veps} : (t,x) \mapsto r_{\veps}^t(t)r_{\veps}^x(x)$. Let $\mu = (\rho,\omega,\zeta)$ be a triplet of measures supported on $\R\times \Omega$ such that $\mu \in \mathcal{CE}_0^1(\rho_0,\rho_1)$, $\mu = (\rho_0,0,0)\otimes \d t$ for $t<0$, and $\mu = (\rho_1,0,0)\otimes \d t$ for $t>1$. Then for all $a\leq-\veps/2$, and $b\geq1+\veps/2$, $\mu \ast r_\veps \in \mathcal{CE}_a^b(\rho_0 \ast r_\veps^x,\rho_1 \ast r_\veps^x)$ on $\Omega+ \bar{B}^d(0,\veps/2)$.
%
\item[Scaling.] Let $\mu = (\rho,\omega,\zeta) \in \mathcal{CE}_a^b(\rho_a,\rho_b)$ with $a<b$ and $T : (t,x) \mapsto (T_t(t), T_x(x))$ be an affine scaling with multiplication factor $\alpha$ and $\beta$, respectively. Then $(\alpha \cdot T_\#\rho, \beta \cdot T_\# \omega,  T_\#\zeta) \in \mathcal{CE}_{T_t(a)}^{T_t(b)}((T_x)_\#(\rho_a),(T_x)_\#(\rho_b))$ on the domain $T_x(\Omega)$.
\end{description}
\end{proposition}


%\todo{Gabriel: I think using $m$ in place of $\rho$ below would be more coherent}

%
\subsection{Action minimizing problems}
In order to select an interpolation among all the solutions to the continuity equation, we choose that which minimizes an \emph{action} functional. A crucial feature of this action which allows to adapt results from classical optimal transport theory is $1$-homogeneity with respect to mass. It is necessary for the model to behave similarly for diffuse and discrete measures. 

Now, two choices of variables are possible. A first approach is to choose a Lagrangian function $L: \Omega \times \R^d \times \R\to \R$ which is a function of the position, the velocity and the rate of growth and to integrate it in space and time to define the action
\begin{equation}\label{eq:actionlagrangian}
\int_0^1 \int_\Omega L(x,v_t(x),g_t(x))\d \rho_t(x),
\end{equation}
which directly generalizes~\eqref{eq:WFInformal}. However, functions built this way are generally not convex even if $L$ is, nor is the continuity equation an affine constraint. This issues are solved if one consider the other set of variables $(\rho,\omega,\zeta)$ because (i) the continuity constraint (Definition~\ref{def:continuity equation}) is affine and (ii) the function $L(x,\omega/\rho,\zeta/\rho)\rho$ is convex and positively $1$-homogeneous if $L$ is convex (this transformation corresponds to taking the \emph{perspective function} of $L$).
%
In the following, we thus directly consider such convex functions of $(\rho,\omega,\zeta)$ that we refer to as \emph{infinitesimal costs}.

%Next, we introduce the admissible class of infinitesimal costs which generalizes the admissible Riemannian inner products defined in Section \ref{sec:AdmissibleMetrics}. 

%Although a standard Lagrangian cost would be defined as a function of the speed $v$ and the growth rate $\alpha$, our infinitesimal cost has nicer analytical properties when defined in terms of the momentum $\omega$ and the source $\zeta$ variables. Indeed, it is then natural to require subadditivity (i.e. we expect that ``locally'', mass is not encouraged to split) and homogeneity in $(\rho,\omega,\zeta)$ (thus convexity). Finally, this change of variables allows interesting costs where $\omega$ or $\zeta$ do not necessarily admit a density w.r.t.\ $\rho$ (see Section \ref{sec:ExamplesPartial} \todo{be more precise in the need}).

\begin{definition}[Infinitesimal cost]
\label{def: infinitesimal cost}
In this paper, an infinitesimal cost is a lower semicontinuous function $f: \Omega \times \R \times \R^d \times \R \to [0,+\infty]$ such that for all $x\in \Omega$, $f(x,\cdot,\cdot,\cdot)$ is convex, positively 1-homogeneous and satisfies
\[
f(x,\rho,\omega,\zeta) 
\begin{cases}
= 0 & \tn{if } (\omega,\zeta) = (0,0) \tn{ and } \rho \geq 0\\
\in ]0,+\infty[ & \tn{if } (\omega,\zeta) \neq (0,0) \text{ and } \rho>0 \\
= + \infty & \tn{if } \rho<0 \, .
\end{cases}
\]
\end{definition}

It is clear that any continuous, convex Lagrangian defines an infinitesimal cost and that reciprocally an infinitesimal cost $f$ defines a continuous, convex Lagrangian $L(x,v,g)= f(x,1,v,g)$ so the two approaches (starting from a Lagrangian or an infinitesimal cost) are in fact equivalent. 

\begin{example}
With the choice of Lagrangian $L(v,g)=\frac12 (|v|^2+g^2)$, the associated infinitesimal cost $f$ is the lower-semicontinuous relaxation of $\frac12 (|\omega|^2/\rho + \zeta^2/\rho)$. This case correspond to the metric $\WF$. We also study in Section~\ref{sec:Examples} Lagrangians of the form $L(v,g)=\frac1p|v|^p+|g|$ with $p>1$, which correspond to the infinitesimal cost $\frac1p |\omega|^p/\rho^{p-1}+|\zeta|$ and show the connection with optimal partial transport.
\end{example}

The dynamic formulation is defined as the minimization of an action defined from the infinitesimal cost $f$.

\begin{definition}[Dynamic problem]
\label{def:DynamicProblem}
For $(\rho,\omega,\zeta) \in \mathcal{M}([0,1] \times \Omega)^{1+d+1}$, let
\begin{align}\label{eq:Jdynamic}
	J_D(\rho,\omega,\zeta) & \eqdef \int_0^1 \int_{\Omega} f(x,\dens{\rho}{\lambda},\dens{\omega}{\lambda},\dens{\zeta}{\lambda})\, \d\lambda(t,x)
%	J_D(\mu) & \eqdef \int_0^1 \int_{\Omega} f(x,\dens{\mu}{|\mu|})\, \d|\mu|(t,x)
	\intertext{where $\lambda \in \mc{M}_+([0,1] \times \Omega)$ is such that $(\rho,\omega,\zeta) \ll \lambda$. Due to 1-homogeneity of $f$, this definition does not depend on the choice of $\lambda$. The dynamic problem is, for $\rho_0,\rho_1 \in \mathcal{M}_+(\Omega)$,}
	\label{eq:dynamic problem}
	C_D(\rho_0,\rho_1) & \eqdef \inf_{(\rho,\omega,\zeta) \in \mathcal{CE}_0^1(\rho_0,\rho_1)} J_D(\rho,\omega,\zeta)\,.
\end{align}
\end{definition}


The expression in~\eqref{eq:Jdynamic} is quite abstract due to the dummy reference measure, which allows to deal correctly with the singular parts of the measures, but it is mainly a rewritting of
~\eqref{eq:actionlagrangian} in terms of the variables $(\rho,\omega,\zeta)$. We will sometimes make the following restrictive assumptions on the infinitesimal cost $f$.

\begin{enumerate}[{(C}1{)}]
\item \emph{multiplicative dependency on $x$}: there exist continuous functions $\lambda_i : \Om \to ]0,+\infty[, \, i\in \{1,\dots , N\}$ such that 
\begin{equation}\label{continuity assumption}
f(x,\rho,\omega,\zeta) = \sum_{i=1}^N \lambda_i(x) \tilde{f}_i(\rho,\omega,\zeta)\, .
\end{equation}
\label{ass: multiplicative}
%where each $\tilde{f}_i$ satisfies an integrability condition: there exists $C_i>0$ such that $|\tilde{f}_i(\cdot)|\leq C_i \max_x f(x,\cdot)$
%
\item \emph{doubling condition}: there exists $C>0$ such that $f(x,\rho,\omega,2\zeta)\leq C \cdot f(x,\rho,\omega,\zeta)$, for all $(x,\rho,\omega,\zeta) \in \Omega \times \R \times \R^d \times \R$.
\label{ass: doubling}
 \end{enumerate}
 %
%Of course, any admissible Riemannian metric from Section 2 defines an infinitesimal cost function which satisfies conditions (C\ref{ass: multiplicative}) and (C\ref{ass: doubling}), by equation \eqref{GeneralFormOfMetric}. 
As is shown in the next result, assumption (C\ref{ass: doubling}) is enough for the dynamic cost $C_D$ to be finite between any pair of nonnegative measures.
%
\begin{proposition}[Finite cost]
\label{prop: finite cost dynamic}
Let $f$ be an infinitesimal cost satisfying assumption (C\ref{ass: doubling}) and such that  $f(x,1,0,1)$ is bounded on $\Omega$. Then for all $(\rho_0,\rho_1)\in \mathcal{M}_+(\Omega)^2$, the dynamic cost \eqref{eq:dynamic problem} is finite, i.e.\ $C_D(\rho_0,\rho_1)< +\infty$.
\end{proposition}
\begin{proof}
Let $C$ be the constant of assumption (C\ref{ass: doubling}) and first assume that $\rho_0=0$. Define, for some $\alpha>0$, the measures $\rho = \rho_1 \otimes (t^\alpha \d t)$, $\omega = 0$ and $\zeta = \rho_1 \otimes (\alpha t^{\alpha-1} \d t)$. By construction $(\rho,\omega,\zeta)\in \mathcal{CE}_0^1(0,\rho_1)$, it only remains to show that for $\alpha$ big enough this triplet has finite cost. By homogeneity of $f$:
\begin{align*}
J_D(\rho,\omega,\zeta) &=
\int_0^1 t^{\alpha} \d t \int_\Omega \d\rho_1 f(x,1,0,\alpha /t)\, .
\end{align*}
By convexity, $f(x,1,0,\cdot)$ increases with the module of the last argument, so with $k(t) := \lceil \log_2(\alpha/t) \rceil$ it holds 
\[
0 \leq f(x,1,0,\alpha/t) \leq f(x,1,0,2^{k(t)}) \leq C^{k(t)} f(x,1,0,1) \leq C' t^{-\log_2 C}
\]
for some $C'>0$ which does not depend on $t$. Consequently, for $\alpha >\log_2 C -1$,
\begin{align*}
C_D(0,\rho_1) \leq J_D(\rho,\omega,\zeta) \leq
C' \int_0^1 t^{\alpha-\log_2 C} \d t \int_\Omega \d\rho_1  < +\infty\, .
\end{align*}
Remark that the preceding argument works as well when reverting or shortening the time interval. Thus, if $\rho_0$ is not the null measure, one builds a interpolation by first decreasing the mass from $\rho_0$ to $0$ for $t\in [0,1/2]$ and then increasing from $0$ to $\rho_1$ for $t\in [1/2,1]$, and the cost of this interpolation is again finite.
\end{proof}
%

\subsection{Properties of dynamic formulations}
The dynamic problem enjoys a dual formulation,  which is the maximization of a linear objective over the set of sub-solutions to a Hamilton-Jacobi equation. Unlike the dual formulation of classical optimal transport, this Hamilton-Jacobi equation involves a term of zeroth order. We state here the proposition in a rather abstract form and explicit examples are given in Section~\ref{sec:Examples}.
%For the definition of lower semicontinuity for set valued functions, see the preliminaries before Theorem \ref{th: duality}.

% DUALITY
\begin{proposition}[Duality]
\label{prop: dynamic dual}
If $f$ is an infinitesimal cost satisfying assumption (C\ref{ass: multiplicative})  then the minimum of \eqref{eq:dynamic problem} is attained. Moreover, denoting $B(x)$ the polar set of $f(x,\cdot,\cdot,\cdot)$ for all $x\in \Omega$, it holds
\begin{equation}
\label{eq: dynamic primal problem}
C_D (\rho_0,\rho_1) = \sup_{\varphi \in K} \int_\Omega \varphi(1,\cdot) \d \rho_1 - \int_\Omega \varphi(0,\cdot) \d \rho_0
\end{equation}
with 
$
K \eqdef \left\{ \varphi \in  C^1([0,1]\times \Omega) : (\partial_t \varphi, \nabla \varphi, \varphi)\in B(x), \, \forall (t,x)\in[0,1]\times \Omega \right\} \, .
$
\end{proposition}

\begin{corollary}[Sublinearity]\label{cor:sublinearityCD}
As the supremum of continuous linear functionals, $C_D$ is a sublinear (i.e.\ convex, positively $1$-homogeneous) and weakly* lower semicontinuous functional.
\end{corollary}

\begin{proof}
Remark, that \eqref{eq: dynamic primal problem} can be written as 
\[
- \inf_{\varphi \in C^1([0,1] \times \Omega)} F(A\varphi) + G(\varphi)
\]
where
$A : \varphi \mapsto (\partial_t \varphi, \nabla \varphi, \varphi)$, is a bounded linear operator from $C^1([0,1]\times \Omega)$ to $C([0,1]\times \Omega)^{d+2}$, and
$F :(\alpha,\beta,\gamma) \mapsto \int_0^1 \int_{\Omega} \iota_{B(x)}(\alpha(t,x),\beta(t,x),\gamma(t,x)) \d x \d t $,
$ G : \varphi \mapsto \int_{\Omega} \varphi(0,\cdot)\d\rho_0 - \int_{\Omega} \varphi(1,\cdot) \d\rho_1$ are convex, proper and lower-semi\-continuous functionals, in particular because for all $x\in \Omega$, the set $B(x)$ is convex, closed and contains $0_{\R^{d+2}}$.
%
Since we assumed that $f(x,\rho,\omega,\zeta)>0$ if $|\omega|>0$ or $\zeta>0$ and $f$ is continuous as a function of $x$ on the compact $\Omega$, one can check that there exists $\veps>0$ such that $(-\veps,0,\theta \epsilon/2) \in \left( \tn{ int } \cap_{x\in \Omega} B(x)\right)$ for $\theta\in [-1,1]$ and thus the function $\varphi : t \mapsto -\veps t +\veps/2$ is such that $F(A\varphi) + G(\varphi)<+\infty$ and $F$ is continuous at $A\varphi$. Then, by Fenchel-Rockafellar duality, \eqref{eq: dynamic primal problem} is equal to
\[
\min_{\mu \in \mathcal{M}([0,1]\times \Omega)^{d+2}}  G^*(-A^*\mu) + F^*(\mu) \, .
\]
By Lemma~\ref{lem:dualitymeasures}, we have $F^*=J_D$, and by direct computations, $G^*\circ (-A^*)$ is the convex indicator of $\mathcal{CE}_0^1(\rho_0,\rho_1)$. 
%For a similar proof strategy with more details see also \cite[Theorem 2.1]{ChizatOTFR2015}.
\end{proof}

The lower-semicontinuity and duality results in this article rely on the following duality property of integral functionals of measures. It is a rephrasing of \cite[Theorem 6]{rockafellar1971integrals} with simplified assumptions thanks to \cite[Lem. A.2]{bouchitte1988integral}.
\begin{lemma}\label{lem:dualitymeasures}
Let $X$ be a compact metric space and $f:X\times\R^n \to \R\cup \{\infty\}$ a l.s.c.\ function such that for all $x\in X$, $f_x(\cdot)=f(x,\cdot)$ is convex, positively $1$-homogeneous and proper. Then $I_f: \mathcal{M}(X)^n\to\R\cup \{\infty\}$ and $I_{f^*}:\mathcal{C}(X)^n\to\R\cup \{\infty\}$ defined as
\[
I_{f}(\mu) \eqdef \int_X f_x(\dens{\mu}{\lambda})\d \lambda 
\quad \text{and}\quad
 I_{f^*}(\phi) \eqdef \begin{cases}
0 &\text{if $\phi(x)\in \mathrm{dom} f(x,\cdot)^*$, $\forall x \in X$},\\
\infty &\text{otherwise}
\end{cases}
\]
form a pair of convex, proper, l.s.c.\ conjugates functions, where the topology considered are the sup-norm topology for $\mathcal{C}(X)^n$ and the weak* topology for $\mathcal{M}(X)^n$. In the definition of $I_f$, $\lambda$ is any nonnegative measure that dominates $\mu$.
\end{lemma}

An important property of these dynamic unbalanced problems is that in many cases they define geodesic distances on the space of nonnegative measures.
\begin{proposition}[Metric property]\label{prop:metricproperty}
Let $f$ be an infinitesimal cost such that $f(x,1,0,1)$ is bounded on $\Omega$. If for all $x\in \Omega$, the function $L_x:(v,g)\mapsto f(x,1,v,g)$ is positively $p$-homogeneous (for some $p>1$) and symmetric with respect to the origin then $C_D^{1/p}$ is a metric and $(\mathcal{M}_+(\Omega),C_D^{1/p})$ is a geodesic metric space.
\end{proposition}
\begin{proof}
Let $\rho_0,\rho_1\in \mathcal{M}_+(\Omega)$. It is clear that $C_D(\rho_0,\rho_1)$ is finite by Proposition \ref{prop: finite cost dynamic}. The symmetry property comes from the symmetry of $L_x$ and the fact that $(\rho,\omega,\zeta)\in \CE_0^1(\rho_0,\rho_1) \Leftrightarrow (\rho,-\omega,-\zeta)\in \CE_0^1(\rho_1,\rho_0)$. It is clear that $C_D(\rho_0,\rho_0)=0$ and conversely, if $C_D(\rho_0,\rho_1)=0$, then $\omega=\zeta=0$ which implies $\rho_0=\rho_1$. Finally, the triangle inequality follows from equation~\eqref{eq:dynalternative} in Lemma~\ref{lem:constantspeed} below, which also proves that any pair of points can be joined by a constant speed minimizing geodesic.
\end{proof}

\begin{lemma}[Constant speed minimizers]\label{lem:constantspeed}
Let $f$ be an infinitesimal cost such that $f(x,1,0,1)$ is bounded on $\Omega$. If for all $x\in \Omega$, the function $L_x:(v,g)\mapsto f(x,1,v,g)$ is positively $p$-homogeneous (for some $p>1$), then minimizers $(\rho,\omega,\zeta)$ of the dynamic problem of Definition~\ref{def:DynamicProblem} can be disintegrated in time w.r.t.\ Lebesgue and satisfy $C_D(\rho_s,\rho_t)=|t-s|C_D(\rho_0,\rho_1)$ for all $0\leq s<t\leq 1$. Moreover, one has for any $T>0$
\begin{equation}\label{eq:dynalternative}
C_D(\rho_0,\rho_1)^{1/p} = \inf \left\{ \int_0^T \left(\int_{\Omega} f(x,\dens{\rho_t}{\lambda_t},\dens{\omega_t}{\lambda_t},\dens{\zeta_t}{\lambda_t})\d \lambda_t \right)^{1/p}\d t\right\}
\end{equation}
where the infimum runs over $(\rho_t,\omega_t,\zeta_t)_{t\in [0,1]}\in \CE_0^T(\rho_0,\rho_1)$ and $\lambda_t$ is a dummy reference measure that dominates $\rho_t,\omega_t$ and $\zeta_t$ for all $t\in [0,T]$.
\end{lemma}
\begin{proof}
By Proposition~ \ref{prop: finite cost dynamic}, we know that $C_D(\rho_0,\rho_1)$ is always finite. Moreover, since $L_x$ is superlinear, any feasible triplet $(\rho,\omega,\zeta)$ satisfies $\omega, \zeta \ll \rho$ from which we can deduce that $\rho$ admits a disintegration in time with respect to the Lebesgue measure on $[0,1]$ (this comes from the fact that $\zeta_t(\Omega)$ is the distributional derivative of $t\mapsto \rho_t(\Omega)$). Let us denote by $\tilde C$ the infimum in~\eqref{eq:dynalternative}, taken with $T=1$ (the fact that this value does not change with $T$ is a consequence of a simple rescaling argument). One may argue exactly as in~\cite[Thm. 5.4]{dolbeault2009new} to show the inequality $C_D\leq\tilde C$. The reverse inequality follows from H\"older inequality and is exact if and only if the integrand equals $C_D(\rho_0,\rho_1)$ $\d t$-a.e.\ for any minimizer $(\rho_t,\omega_t,\zeta_t)_{t\in [0,1]}$. This constant speed property, combined with the fact that $(\rho,\omega,\zeta)$, after time rescaling, remains minimizing between any pair of intermediate times $0\leq s<t\leq1$ (otherwise one could improve the action on $[0,1]$ by glueing), leads to the constant speed property.
\end{proof}


The main goal of this article is to formulate a Kantorovich-like formulation for problems of this kind. This aim requires to introduce a new definition of \emph{static} optimal transport problems, and this is the object of the next section. The relationship between these two classes of models is stated and proved in Section~\ref{sec:DynamicToStatic}.



==> Submission Final JFA/Dynamic2static.tex <==
% !TEX root = ../DynamicToStatic.tex

%%%%%%%%%%%%%%%%%%%%%%%%%
% DYNAMIC
%%%%%%%%%%%%%%%%%%%%%%%%%

\section{From Dynamic to Static Problems}
\label{sec:DynamicToStatic}
In the previous sections, we have introduced and studied basic properties of two categories of unbalanced optimal transport problems: dynamic formulations and semi-coupling formulations. In this section, we prove (Theorem~\ref{th: continuous static general}) that any dynamic problem is equivalent to a semi-coupling problem. We put ourselves back in the setting of Section~\ref{sec:dynamic} where $\Omega$ is the closure of an open, connected, bounded subset of $\R^d$ with Lipschitz boundary.

%In this section we establish that a certain class of convex, positively homogeneous, optimization problems over the solutions of the continuity equation with source (informally introduced in \ref{eq:ContinuityEqInformal}) --- the dynamic problems --- admits unbalanced Kantorovich formulations that we introduced in Sect.\ \ref{sec : general static problem} --- the static problems. We prove an equivalence result between static and dynamic models for a large class of dynamic models.
%\subsection{Connection Between Static and Dynamic Problems}

%Theorem~\ref{th: continuous static general} is the main result of this section. It states that if the cost $c$ of the static problem is defined as the dynamic cost between Diracs, then the static and the dynamic formulations coincide. 
%
%The cost $c$ of the static problem can alternatively be determined as a generalized action on the paths space as measured by an infinitesimal cost $f$ (see Proposition \ref{prop : alternative dynamic/static}).
%
%In the Riemannian setting this means that $c$ is the squared geodesic distance on $\Cone(\Omega)$, see Sect.~\ref{sec:AdmissibleMetrics}.
%
%Of course, there are static costs $c$ that do not arise from a dynamic cost $f$, just as there are dynamic problems beyond the framework of Definition \ref{def: infinitesimal cost} which cannot be cast into a static form.

% The cost $c$ of the static problem is determined by the dynamic formulation \eqref{eq: dynamic primal problem} as a generalized action on the path space. In the case where $f$ gives rise to a Riemannian metric on $\Omega \times \R_+^*$, $c$ is simply the square of the distance associated with the metric. This is detailed in the following theorem.

\subsection{Minimal path cost and convexification}

\iffalse
\begin{definition}
The Dirac-based cost is
\begin{align}
	\label{eq:c between Diracs}
	c_d : (x_0, m_0) , (x_1, m_1) \mapsto C_D(m_0 \delta_{x_0}, m_1 \delta_{x_1}) \, .
\end{align}
If $c_d$ is lower-semicontinuous, then it defines a \emph{cost function}. 
\end{definition}
\fi

Any infinitesimal cost $f$ defines a cost function on $\Omega \times \R_+$ obtained by minimizing over absolutely continuous trajectories.

\begin{definition}[minimal path cost]
The minimal path cost associated to the Lagrangian $L$ is, for $(x_i,m_i)\in \Omega\times\R_+$ with $i\in \{0,1\}$,
\begin{equation}\label{eq-pathspace}
c_f(x_0,m_0,x_1,m_1) \eqdef \inf_{ x(t),m(t)}  \int_0^1 f(x(t),m(t),m(t)\, x'(t),m'(t)) \, \d t\,
\end{equation}
where the infimum runs over absolutely continuous paths $t\mapsto(x(t),m(t))$ that link $(x_0,m_0)$ to $(x_1,m_1)$.
%for $(x(t),m(t)) \in C^1([0,1],\Omega \times [0,+\infty[)$ such that $(x(i),m(i)) = (x_i,m_i)$ for $i\in \{ 0,1\}$.
\end{definition}

In general, $c_f$ does not define a cost function in the sense of Definition \ref{def:CostFunction} because of a possible lack of convexity, but its convex regularization does so. This convex relaxation can be nicely expressed as the minimal path cost obtained by allowing mass to be split in two ``travelling'' Dirac masses.

\begin{proposition}[properties and convexification]\label{prop : alternative dynamic/static}
Assume that properties C\ref{ass: multiplicative} and C\ref{ass: doubling} hold for the infinitesimal cost $f$. Then the minimal path cost $c_f$ is finite and continuous on $(\Omega\times\R_+)^2$. Morevoer, its convex regularization $\tilde c_f$ is an admissible cost function, is continuous, and characterized by
\begin{equation}\label{eq:c one or two diracs}
\tilde c_f(x_0,m_0,x_1,m_1 ) = \min_{\substack{m_0^a+m_0^b=m_0\\m_1^a+m_1^b=m_1}} c_f(x_0,m_0^a,x_1,m_1^a)+ c_f(x_0,m_0^b,x_1,m_1^b)\, .
\end{equation}
\end{proposition}
\begin{proof}
The argument of the proof of Proposition~\ref{prop: finite cost dynamic} shows that $c_f$ is finite on its domain. It is also continuous since one can perturb a path and reach nearby points with a perturbed cost (thanks to assumption C\ref{ass: multiplicative}). As for $\tilde c_f$, it is clear that it takes values in $[0,\infty]$ and that it inherits $1$-homogeneity from $f$, so $\tilde c_f(x,\cdot,y\cdot)$ is sublinear for all $(x,y)$. Moreover, characterization is a consequence of Carath\'eodory's Theorem \cite[Corollary 17.1.6]{rockafellar2015convex} (one can also check directly that is it valid for $(m_0,m_1)=(0,0)$ although this is not part of the cited result). The infimum is attained because $c_f$ is continuous and the minimization set is compact. Finally, the continuity of $\tilde c_f$ is clear from this characterization and the continuity of $c_f$.
\end{proof}
%
\iffalse
The next proposition gives a sufficient condition for $c_s$ to be finite when $\Omega$ is convex (for simplicity).
%
\begin{proposition}
If $\Omega \subset \R^d$ is convex and $f$ is an infinitesimal cost which satisfies assumptions (C\ref{ass: multiplicative}) and (C\ref{ass: doubling}) , then for all $(x_0,x_1)\in \Omega^2$ and $(m_0,m_1)\in [0,+\infty[^2$, $c_s(x_0,m_0, x_1,m_1)$ is finite.
\end{proposition}
\begin{proof}
If $m_0=0$ (or similarly if $m_1=0$), then the smooth trajectory $(x_1,t^\alpha m_1)$ has a finite cost for $\alpha>0$ big enough (see the proof of Prop. \ref{prop: finite cost dynamic}). 
%
If $m_0>0$ and $m_1>0$ then the smooth interpolation $(x(t),m(t))=(x_0 + t v, m_0\cdot e^{\alpha t})$ with $v= x_1-x_0$ and $\alpha = \log(m_1/m_0)$  satisfies $(x(i),m(i))=(x_i,m_i)$ for $i\in \{0,1\}$ and by homogeneity,
\[
\int_0^1 f(x(t),m(t),m(t)x'(t),m'(t))\d t = \int_0^1 f(x(t),1,v,\alpha) m(t) \d t < +\infty\, .
\]
\end{proof}
\fi

%This convexification is a crucial step and it is $\tilde c_f$ that plays the main role in the 

%Note that in general, $\tilde c_f\neq c_f$, since, as opposed to the dynamic problem $C_D$, the problem defining $c_s$ is not allowed to split mass. For instance, we will see in Section \ref{sec:equivalence WF} that the cut distance is $\pi/2$ for the $\WF$ metric while it is $\pi$ for the associated minimal path cost.

\subsection{Main Theorem}

We can now state our main theorem, which connects the dynamic and the semi-coupling formulations of unbalanced optimal transport.

\begin{theorem}
\label{th: continuous static general}
Let $\Omega \subset \R^d$ be a compact which is star shaped w.r.t.\ a set of points with nonempty interior, and $f$ be an infinitesimal cost satisfying (C\ref{ass: multiplicative})  and (C\ref{ass: doubling}). Defining $\tilde c_f$ the convex relaxation of the minimal path cost (as in Proposition~\ref{prop : alternative dynamic/static}) as the static cost, it holds, for $\rho_0, \rho_1 \in \mathcal{M}_+(\Omega)$, 
\[
C_D(\rho_0, \rho_1) = C_K(\rho_0,\rho_1).
\]
\end{theorem}
%
%\begin{theorem}\label{th: continuous static general}
%Let $\Omega \subset \R^d$ be a compact which is star shaped w.r.t.\ a set of points with nonempty interior, and $c$ be a cost function satisfying $c_d \leq c \leq c_s$, where $c_d$ and $c_s$ are derived from an infinitesimal cost $f$ satisfying (C\ref{ass: multiplicative})  and (C\ref{ass: doubling}). If the associated static problem $C_K$ is weakly* continuous,\todo{useless} it holds, for $\rho_0, \rho_1 \in \mathcal{M}_+(\Omega)$, $C_D(\rho_0, \rho_1) = C_K(\rho_0,\rho_1)\,$ and $c = c_d$.
%\end{theorem}
%
The assumption on the domain includes convex sets but also most star-shaped sets. This particular assumption comes from the fact that our proof strategy involves a smoothing step that needs to deal correctly with the dependency in $x$ of the infinitesimal cost $f$.

%In general, computing $c_d$ directly is not easy : the margin in the choice of $c$ in Theorem \ref{th: continuous static general} allows to obtain $c_d$ as a consequence of the Theorem, not as a requirement. A natural choice for $c$ is the convex regularization of the cost on the path space $c_s$, which is easier to compute than $c_d$. It can be nicely expressed as the optimal cost on the path space when allowing the Dirac to be split into two chunks:
%
\iffalse
\begin{proposition}
\label{prop : alternative dynamic/static}
The convex regularization of $c_s$ can be expressed as
\begin{equation}\label{eq:c one or two diracs}
\tilde c_s : (x_0,m_0) , (x_1,m_1 ) \mapsto \inf_{\substack{m_0^a+m_0^b=m_0\\m_1^a+m_1^b=m_1}} c_s(x_0,m_0^a,x_1,m_1^a)+ c_s(x_0,m_0^b,x_1,m_1^b)\, .
\end{equation}
It is convex, positively homogeneous in $(m_0,m_1)$, and $c_d \leq \tilde c_s \leq c_s$.
\end{proposition}

\begin{proof}%[Proof of Corollary \ref{cor : alternative dynamic/static}]
The fact that \eqref{eq:c one or two diracs} is the convex regularization of $c_s$ is a consequence of Carath\'eodory's Theorem \cite[Corollary 17.1.6]{rockafellar2015convex}. In particular, $\tilde c_s \leq c_s$.  
%
For the other inequality, consider an admissible splitting of the mass $(m_0^a,m_0^b,m_1^a,m_1^b)$.  Candidate solutions $(\rho,\omega,\zeta)$ for the dynamic problem \eqref{def:DynamicProblem} are built by taking the sum of two travelling Dirac masses, with smooth speeds and variation of masses, one linking $m_0^a \delta_{x_0}$ to $m_1^a \delta_{x_1}$ and the other linking $m_0^b \delta_{x_0}$ to $m_1^b \delta_{x_1}$. Minimizing over this class of trajectories, one recovers by linearity of \eqref{def:DynamicProblem} and the definition of $c_s$ that 
\[
c_d(x_0,m_0,x_1,m_1) \leq c_s(x_0,m^a_0,x_1,m^a_1) + c_s(x_0,m^b_0,x_1,m^b_1) \, .
\]
Since this is true for any splitting of mass, it holds $c_d \leq \tilde c_s$, which concludes the proof.
\end{proof}
\fi
% We now proceed to the proof of Theorem \ref{th: continuous static general}.

%
\begin{proof}[Proof of Theorem \ref{th: continuous static general}]
%It is clear that $c_d\leq c_s$ because for any candidate path $(x(t),m(t))$ in \eqref{eq-pathspace}, $m(t)\delta_{x(t)} \otimes \d t \in \mathcal{CE}_0^1(m_0 \delta_{x_0}, m_1 \delta_{x_1})$, and thus the assumption $c_d \leq c \leq c_s$ is not void. 
The proof is divided into three steps: in Step 1, we show, using discrete approximations of semi-couplings, that it holds $C_K\geq C_D$. By integrating characteristics (an argument similar to the original proof of the Benamou-Brenier formula \cite{benamou2000computational}), we show in Step 2 that for absolutely continuous marginals, $C_K$ is upper bounded by the dynamic minimization problem restricted to smooth fields. In Step 3, a regularization argument, inspired by \cite[Theorem 8.1]{cedric2003topics}, extends this result to general measures and shows that $C_K\leq C_D$. %The conclusion, in Step 4, follows by a density argument. %It can be checked that $\tilde c_f$ satisfies the assumptions of Theorem \ref{th : continuity continuous static} which implies that %For clarity, we write $c$ for $\tilde c_f$ in the proof.

\paragraph{Step 1.}
Let $(\rho_0,\rho_1)\in \mathcal{M}_+(\Omega)^2$ and %let $(f \gamma,g \gamma)$ be an optimal pair of semi-couplings for $C_{h}(\mu,\nu)$, where $ \gamma \in \P(\Omega^2)$ and $f,g \in L^1( \gamma)$.  
%
let $(\hat \gamma_0^{(n)})$, let $(\hat \gamma_1^{(n)})$ be the atomic measures on $\Omega^2$ given by Lemma \ref{lem:approximationsemicoupling} below (the continuity of $h$ follows from Proposition \ref{prop : alternative dynamic/static}): they are such that  $\lim_{n\to \infty} J_K(\hat \gamma_0^{(n)},\hat \gamma_1^{(n)}) = C_K(\rho_0,\rho_1)$. Also denote by $(\rho_0^n,\rho_1^n)\eqdef((\Proj_0)_\# \bar \gamma^{(n)}_0,\allowbreak (\Proj_1)_\# \bar \gamma^{(n)}_1)$ the corresponding marginals, that satisfy $\rho_0^n\rightharpoonup^* \rho_0$ and $\rho_1^n\rightharpoonup \rho_1$. 

From the definition of $c_f$ and by characterization \eqref{eq:c one or two diracs} of $\tilde c_f$ one has that $\tilde c_f(x_0,m_0,x_1,m_1)\geq C_D(m_0\delta_{x_0},m_1\delta_{x_1})$. It follows, taking the notations of the proof of Lemma \ref{lem:approximationsemicoupling},
\begin{align*}
J_K(\hat \gamma_0^{(n)},\hat \gamma_1^{(n)})
&= \sum_{i\in I} \tilde c_f(x_i, f^{(n)}_i,y_i,g^{(n)}_i)\gamma_i^{(n)}\\
&\geq \sum_{i\in I} C_D(f^{(n)}_i  \gamma_i^{(n)} \delta_{x_i}, g^{(n)}_i  \gamma_i^{(n)} \delta_{y_i}) \geq C_D(\rho_0^n,\rho_1^n).
\end{align*}
Since by Corollary~\ref{cor:sublinearityCD}, $C_D$ is weakly l.s.c., it follows $C_D(\mu,\nu)\leq C_K(\mu,\nu)$.


\iffalse 
For the static problem $C_K$, there exists a minimizer in the set $\Gamma(\rho_0,\rho_1)\cap \mathcal{M}_+^{at}(\Omega^2)^2$. Indeed, an atom assigned to another atom is represented by an atom in $\Om^2$, and the same can be forced to hold for an atom assigned to the apex, because for all $x\in \Omega$, $\tilde c_f(x,1,\cdot,0)$ attains its minimum in $\Omega$. Let $(\gamma_0,\gamma_1)$ be such a minimizer, it can be written $\gamma_k = \sum_{i,j} m^k_{i,j} \delta_{(x_i,x_j)}$, for $k=0,1$. From the definition of $c_f$ and by characterization \eqref{eq:c one or two diracs} of $\tilde c_f$ one has that $\tilde c_f(x_0,m_0,x_1,m_1)\geq C_D(m_0\delta_{x_0},m_1\delta_{x_1})$. As a consequence, it holds
\begin{align*}
C_K(\rho_0,\rho_1) 
&= \sum_{i,j} \tilde c_f(x_i,m^0_{i,j},x_j,m^1_{i,j})\\
&\geq \sum_{i,j} C_D ( m^0_{i,j} \delta_{x_i} , m^1_{i,j} \delta_{x_j})\\
& \geq C_D \big(\sum_{i,j} m^0_{i,j} \delta_{x_i} , \sum_{i,j} m^1_{i,j} \delta_{x_i}\big) = C_D(\rho_0,\rho_1)
\end{align*}
where for the last inequality we used the fact that $C_D$ is subbadditive: it is indeed defined as the infimum of the subbaditive functional $J_D$ (which inherits subadditivity from the infinitesimal cost $f$) under linear constraints.
\fi



\paragraph{Step 2.} Let $\rho_0,\, \rho_1 \in  \mathcal{M}_+(\Omega)$ be absolutely continuous measures with positive mass and let
\[
(\rho,\omega,\zeta) \in \left\{ (\rho,\omega,\zeta)\in \mathcal{CE}_0^1(\rho_0,\rho_1) : \dens{\omega}{\rho}, \dens{\zeta}{\rho}\in C^1([0,1]\times \Omega) \right\} \, .
\]
%and define $C_D^{sm} \eqdef \inf_{\mathcal{CE}_{sm}(\rho_0,\rho_1)} J_D(\rho,\omega, \zeta)$.
%
%
One can take the Lagrangian coordinates $(\varphi_t(x),\lambda_t(x))$ which are given by the flow of the smooth fields $(v\eqdef \omega/\rho, g \eqdef \zeta/\rho)$ (see \cite[Prop. 3.6]{maniglia2007probabilistic}) :
\begin{align*}
\partial_t \varphi_t(x) = v_t(\varphi_t(x)) \quad \tn{and} \quad
\partial_t  \lambda_t(x) = g_t(\varphi_t(x))\lambda_t(x) \, ,
\end{align*}
with the initial condition $(\varphi_0(x), \lambda_0(x)) = (x,1)$. The Neumann boundary conditions on $v$, included in the continuity equation, imply that for all $t\in [0,1]$, $\Omega$ is stable by $\varphi_t$. Recall that $(\varphi_t(x),\lambda_t(x))$ describes the position and the relative increase of mass at time $t$ of a particle initially at position $x$ and that one has $\rho_t = (\varphi_t)_\# (\lambda_t \cdot \rho_0)$.
%
It follows
\begin{align*}
J_D(\rho,\omega, \zeta) 
&= \int_{[0,1] \times \Omega} f\big(x,1,v_t(x),g_t(x)\big) \d[(\varphi_t)_{*} \big(\lambda_t \rho_0 \big)](x) \d t \\
&\overset{(1)}{=} \int_{\Omega} \left[ \int_0^1 f\big(\varphi_t(x),1, \partial_t \varphi_t(x), \partial_t \lambda_t(x)/\lambda_t(x) \big) \lambda_t(x) \d t \right] \d \rho_0(x) \\
&\overset{(2)}{=}  \int_{\Omega} \left[ \int_0^1 f\big(\varphi_t(x),\lambda_t(x), \lambda_t(x) (\partial_t \varphi_t(x)),\partial_t \lambda_t(x) \big) \d t \right] d \rho_0(x) \\
&\overset{(3)}{\geq} \int_{\Omega} c_f(x,1, \varphi_1(x), \lambda_1(x)) d \rho_0(x) \\
&\overset{(4)}{\geq}  C_K(\rho_0,\rho_1)
\end{align*}
where we used (1) the change of variables formula (2) homogeneity of $f$ (3) the definition of the minimal path cost $c_f$ and (4) 
the fact that  $\big( \pfwd{(\id, \varphi_1)} \rho_0, \allowbreak \pfwd{(\id, \varphi_1)} (\lambda_1 \rho_0)\big)\in \Gamma(\rho_0,\rho_1)$ and $c_f\geq \tilde c_f$.
%\end{proof}
%
%\begin{lemma}
%\label{lemma : smoothing argument}
\paragraph{Step 3.} 
Let $\rho_0, \rho_1 \in \mathcal{M}_+(\Omega)$. We want to show, with the help of Step 2, that $C_K(\rho_0, \rho_1) \leq C_D(\rho_0, \rho_1)$.
%\end{lemma}
%\begin{proof}
Let $(\rho,\omega,\zeta) \in \mathcal{CE}_0^1(\rho_0,\rho_1)$ and for $\delta \in ]0,1[$ let
\[
\tilde{\rho}^{\delta} = (1-\delta) \rho + \delta\, (\d x \otimes \d t)\vert_{S}, \quad \tilde{\omega}^{\delta} = (1-\delta) \omega, \quad \tilde{\zeta}^{\delta} = (1-\delta) \zeta
\]
where $S\supset \Omega$ is a bounded set containing $\Omega+B^d(0,1)$ and $B^d(a,r)$ denotes the open ball of radius $r$ centered at point $a$ in $\R^d$. One has $(\tilde{\rho}^{\delta} ,  \tilde{\omega}^{\delta}, \tilde{\zeta}^{\delta} )\vert_\Omega \in \mathcal{CE}_0^1(\tilde{\rho}_0^{\delta}\vert_\Omega,\tilde{\rho}_1^{\delta}\vert_\Omega)$ and by convexity, 
\[
J_D(\tilde{\rho}^{\delta} ,  \tilde{\omega}^{\delta}, \tilde{\zeta}^{\delta} ) \leq J_D(\rho, \omega, \zeta)\, .
\]
Since $\tilde{\rho}_0^{\delta}\vert_\Omega \rightharpoonup^*\rho_0$ and $\tilde{\rho}_1^{\delta}\vert_\Omega \rightharpoonup^*\rho_1$ as $\delta \to 0$ and $C_K$ is weakly* lower semicontinuous (Corollary~\ref{cor:sublinearityCK}), it is sufficient to prove
$
J_D(\tilde{\rho}^{\delta} ,  \tilde{\omega}^{\delta}, \tilde{\zeta}^{\delta} ) \geq C_K(\tilde{\rho}_0^{\delta}\vert_{\Omega} ,  \tilde{\rho}_1^{\delta}\vert_\Omega ) 
$
for proving $J_D(\rho, \omega, \zeta) \geq C_K(\rho_0,\rho_1)$.
%
In order to alleviate notations we shall now denote $\tilde{\rho}^{\delta} ,  \tilde{\omega}^{\delta}, \tilde{\zeta}^{\delta} $ by just $\rho, \omega, \zeta$ and the new marginals $\tilde{\rho}_0^{\delta},  \tilde{\rho}_1^{\delta}$ by $\rho_0,\rho_1$ (now supported on $S\supset \Omega$).
%
Up to a translation, we can assume that $0$ is in the interior of the set of points w.r.t.\ which $\Omega$ is star shaped. Then \cite[Theorem 5.3]{rubinov2013abstract} tells us that the Minkowski gauge $x \mapsto \inf \{ \lambda>0 : x \in \lambda \Omega \}$ is Lipschitz: let us denote by $k\in \R_+^*$ its Lipschitz constant.
%
We introduce the regularizing kernel
$
r_{\veps}(t,x) = \frac{1}{\veps^{d}}\, r_1\left( \frac{x}{\veps} \right) \frac{1}{\veps}\, r_2 \left( \frac{t}{\veps} \right) \, 
$
where $r_1 \in C_c^{\infty}(B^d(0,\frac{1}{2k}))$, $r_2 \in C_c^{\infty}(B^1(0,\frac{1}{2k}))$, $r_i \geq 0$, $\int r_i = 1$, $r_i$ even ($i=1,2$). We want to perform a smoothing procedure which, in some sense, preserves the domain $\Omega$ because this is where $f$ and $\tilde c_f$ are defined.

Let $\bar{\mu}=((1+\veps)^{-1}\bar{\rho},(1+\veps)^{-1}\omega,\zeta)$ where $\bar{\rho}$ is a measure on $[-\veps,1+\veps]\times S$ which is worth $\rho$ on $[0,1]\times S$,  $\rho_0 \otimes \d t$ on $[-\veps,0[\times S$ and $\rho_1 \otimes \d t$ on $]1,1+\veps]\times S$ (while $\omega, \zeta$ are always implicitely extended by $0$). 
%By the extension property in Proposition \ref{prop:results on continuity equation}, $(\bar{\rho},\omega,\zeta)$ still satisfies the continuity equation.
Then define
\[
\mu^\veps \eqdef T_{\#} (\bar{\mu} \ast r_\veps)\vert_{[0,1]\times \Omega},
\]
where $T:(t,x) \mapsto ((1+\veps)^{-1}(t+ \veps/2),(1+\veps)^{-1}x)$ is built in such a way that the image of the time segment $[-\veps/2,1+\veps/2]$ is $[0,1]$. Furthermore, since the Minkowski gauge of $\Omega$ is $k$-Lipschitz, the image of $\Omega^\veps \eqdef \Omega + B^d(0,\veps/k)$ by $T$ is included in $\Omega$. Now, by the smoothing and scaling properties in Proposition \ref{prop:results on continuity equation}, it holds $\mu^{\veps} \in \mathcal{CE}_0^1(\rho^{\veps}_0,\rho^{\veps}_1)$ for some smoothed marginals $(\rho_0^\veps, \rho_1^\veps)$.
%  in particular because we took care of multiplying $\rho$ and $\omega$ by a factor $(1+\veps)^{-1}$ in the definition of $\bar{\mu}$. 

Notice that $\rho^{\veps}_0 \rightharpoonup^* \rho_0\vert_\Omega$ and $\rho^{\veps}_1 \rightharpoonup^* \rho_1\vert_\Omega$ when $\veps \to 0$ since these measures are the evaluations of $\bar{\mu}\ast r_\veps$ at time $-\veps/2$ and $1+\veps/2$, respectively (also contracted in space by a factor $1+\veps$ and restricted to $\Omega$). Moreover, the vector fields $\omega_t^{\veps}/ \rho_t^{\veps}$ and $\zeta_t^{\veps}/ \rho_t^{\veps}$ are well-defined, smooth, bounded functions on $[0,1]\times \Omega$ because $\rho^\veps$ has a density bounded from below by a positive constant whenever $\veps/k <1$ (so that $\Omega^\veps\subset S$). Therefore, by Step 2,
\[
J_D(\mu^{\veps}) \geq C_K(\rho_0^{\veps}, \rho_1^{\veps}).
\]
On the other hand, for any $\veps'>0$, one has
\begin{align*}
J_D(\mu^{\veps}) 
& =  \int_0^1 \int_{\Omega} f(y, \dens{\mu^{\veps}}{|\mu^{\veps}|}) \d |\mu^{\veps}|(s,y)  \\
& \overset{(1)}{=}  \int_{-\veps/2}^{1+\veps/2} \int_{\Omega^\veps} f((1-\veps)y, \dens{\bar{\mu} \ast r_{\veps}}{|\bar{\mu} \ast r_{\veps}|}) \d |\bar{\mu}\ast r_{\veps}|(s,y) \\
& \overset{(2)}{\leq}  \int_{-\veps/2}^{1+\veps/2} \int_{\Omega^\veps} \d |\bar{\mu}|(t,x) \int_{\R^{1+d}} \!\!\! \d s \d y f((1-\veps)y, \dens{\bar{\mu}}{|\bar{\mu}|}(t,x)) \cdot r_{\veps}(s-t,y-x)  \\
&  \overset{(3)}{=}  \sum_i \int_{0}^{1} \int_{\Omega} \d |\bar{\mu}|(t,x) \int_{\R^{1+d}} \!\!\! \d s \d y \tilde{f}_i(\dens{\bar{\mu}}{|\bar{\mu}|}(t,x))   \lambda_i((1-\veps)y) r_{\veps}(s-t,y-x)  \\
& \overset{(4)}{\leq} \int_0^{1} \int_{\Omega} (1+\veps')f(x, \dens{\bar{\mu}}{|\bar{\mu}|})  \d |\bar{\mu}|(t,x) 
\end{align*}
where were used (1) the change of variable formula, (2) the convexity and homogeneity of $f$, (3) assumption (C\ref{ass: multiplicative})  (which also garanties the integrability of each $\tilde{f}_i$) assumed on $f$ and (4) the continuity of the strictly positive factors $(\lambda_i)_i$, if for a given $\veps'>0$, one choses $\veps$ small enough. Therefore $ J_D(\bar{\mu}) \geq J_D(\mu^\veps)(1+\veps')^{-1}$. But by convexity and homogeneity, $J_D(\bar{\mu})\leq (1+\veps)^{-1} ((1-\veps)J_D(\rho,\omega,\zeta) + \veps J_D(\rho,\omega,2\zeta))$. By the ``doubling'' assumption (C\ref{ass: doubling})  on $f$, the term $J_D(\rho,\omega,2\zeta)$ is finite if $J_D(\rho,\omega,\zeta)$ is finite and one has
\[
C_K(\rho_0^{\veps}, \rho_1^{\veps}) \leq \frac{1+\veps'}{1+\veps}((1-\veps)J_D(\rho,\omega,\zeta) + \veps J_D(\rho,\omega,2\zeta))\, .
\]
%
Letting $\veps'$ and $\veps$ go to $0$, using the lower semicontinuity of $C_K$ and taking the infimum, one recovers in the end $C_K(\rho_0\vert_\Omega,\rho_1\vert_\Omega) \leq J_D(\rho,\omega,\zeta)$ as desired.
%\end{proof}
%\paragraph{Step 4.}
%We have proven in Step 1 that if  $\rho_0, \rho_1 \in \mathcal{M}_+^{at}(\Omega)$, then
%\[C_D(\rho_0, \rho_1) \leq C_K (\rho_0, \rho_1)\, .\]
%Moreover, by Step 3, for all $\rho_0, \rho_1 \in \mathcal{M}_+(\Omega)$ on has
%\[C_D (\rho_0, \rho_1)\geq C_K(\rho_0, \rho_1) \, .\]
%and thus $C_D=C_K$ for atomic measures.  But $C_D$ is weakly* l.s.c since $J_D$ is lower semicontinuous by Lemma \ref{lem:dualitymeasures}. Finally, by density of $\mathcal{M}_+^{at}(\Omega)$ in $\mathcal{M}_+(\Omega)$, for $\rho_0, \rho_1 \in \mathcal{M}_+(\Om)$, $C_D(\rho_0, \rho_1)\leq C_K(\rho_0, \rho_1)$. %The equality $c=c_d$ is direct by computing $C_K$ between Dirac measures, and because $c$ is subadditive.
\end{proof}


\begin{lemma}[Atomic approximation of semi-couplings]\label{lem:approximationsemicoupling}
Let $\mu\in \mathcal{M}_+(\Omega)$ and $\nu\in \mathcal{M}_+(\Omega)$. If $c$ is a continuous cost function, then there exists a sequence of finitely atomic measures $(\gamma_0^{(n)})$ and $(\gamma_1^{(n)})$ that weakly converge to an optimal pair of semi-couplings for $C_K(\mu,\nu)$ and such that 
\[
\lim_{n\to \infty} J_K(\gamma_0^{(n)},\gamma_1^{(n)}) = C_K(\mu,\nu).
\]
\end{lemma}
\begin{proof}
Let $(f \gamma,g \gamma)$ be an optimal pair of semi-couplings for $C_K(\mu,\nu)$, where $ \gamma \in \M_+(\Omega^2)$ and $f,g \in L^1( \gamma)$. Let $(B^{(n)}_i, (x_i,y_i)^{(n)})_{i\in I}$ be sequence of finite pointed partitions of $\Omega^2$ such that $\lim_{n\to \infty}\max_{i\in I} \diam \, B^{(n)}_i=0$.  We define the discrete approximations $\bar \gamma_0^{(n)}\eqdef T^{(n)}_\# (f\gamma)$ and $\bar \gamma_1^{(n)}\eqdef T^{(n)}_\# (g\gamma)$ where $T^{(n)}:\Omega^2\to \Omega^2$ maps all points in $B_i^{(n)}$ to $(x_i,y_i)^{(n)}$.
Also, denote $(\Proj_0)_\# \bar \gamma^{(n)}_0 =\mu_n$ and $(\Proj_1)_\# \bar \gamma^{(n)}_1=\nu_n$.
 It is clear that the discretized semi-couplings weakly converge to $(f\gamma,g\gamma)$. Moreover, for $\epsilon>0$, there exists $n\in \N$ such that for all $i\in I$, by Jensen inequality, and since $c$ is continuous, uniformly on $(X\times [0,1])\times (Y \times [0,1])$,
\begin{multline*}
c(x_i^{(n)},\bar \gamma_0^{(n)}(B_i^{(n)}),y_i^{(n)}, \bar \gamma_1^{(n)}(B_i^{(n)})) \leq \epsilon \max\{\bar \gamma_0^{(n)}(B_i^{(n)}),\bar \gamma_1^{(n)}(B_i^{(n)})\} \\ 
+ \int_{B^{(n)}_i} c(x,f(x,y),y,g(x,y))\d \gamma(x,y)
\end{multline*}
%\[h_{(x_i,y_i)^{(n)}}(f^{(n)}_i,g^{(n)}_i)\gamma_i^{(n)} \leq \eps \gamma_i^{(n)}+ \int_{B^{(n)}_i} h_{x,y}(f\gamma,g\gamma) \]
By integrating on the whole domain, one has
\[
J_K(\hat \gamma_0^{(n)},\hat \gamma_1^{(n)}) \leq  \epsilon\cdot (\mu(X)+\nu(Y)) + C_h(\mu,\nu)
\]
and the result follows because $\epsilon$ can be arbitrarily small.
\end{proof}



==> Submission Final JFA/Introduction.tex <==
% !TEX root = ../DynamicToStatic.TEX

\section{Introduction}

Optimal transport is an optimization problem which gives rise to a popular class of metrics between probability distributions. We refer to the monograph of Villani~\cite{cedric2003topics} for a detailed overview of optimal transport. 
%
A major constraint of the resulting transportation metrics is that they are restricted to measures of equal total mass (e.g.\ probability distributions). In many applications, there is however a need to compare unnormalized measures, which corresponds to so-called \emph{unbalanced} optimal transport problems, following the terminology introduced in~\cite{benamou2003numerical}. Applications of these unbalanced metrics range from image classification~\cite{rubner1997earth,pele2008linear} to the processing of neuronal activation maps~\cite{GramfortMICCAI}.
%
This class of problems requires to precisely quantify the amount of transportation, creation and destruction of mass needed to compare arbitrary positive measures. While several proposals to achieve this goal have been made in the literature (see below for more details), to the best of our knowledge, there lacks a coherent framework that enables to deal with generic measures while preserving both the dynamic and the static perspectives of optimal transport. It is precisely the goal of the present paper to describe such a framework and to explore its main properties. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Previous work}
In the last few years, there has been an increasing interest in extending optimal transport to the unbalanced setting of measures having non-equal masses. 
%%%
\paragraph{Dynamic formulations of unbalanced optimal transport. }

Several models based on the fluid dynamic formulation introduced in~\cite{benamou2000computational} have been proposed recently~\cite{OTmaasrumpf,lombardi2013eulerian,piccoli2014generalized,piccoli2013properties}. In these works, a source term is introduced in the continuity equation. They differ in the way this source is penalized or chosen.
%
We refer to~\cite{ChizatOTFR2015} for a detailed overview of these models.  

%%%
\paragraph{Static formulations of unbalanced optimal transport. }
Purely static formulations of unbalanced transport are however a longstanding problem. 
%
A simple way to address this issue is given in the early work of Kantorovich and Rubinstein~\cite{kantorovich1958space}. The corresponding ``Kantorovich norms'' were later extended to separable metric spaces by~\cite{hanin1999extension}. These norms handle mass variations by allowing to drop some mass from each location with a fixed transportation cost. 
%
The computation of these norms can in fact be re-casted as an ordinary optimal transport between normalized measures by adding a point ``at infinity'' where mass can be sent to, as explained by~\cite{guittet2002extended}. This reformulation is used in~\cite{GramfortMICCAI} for applications in neuroimaging. 
%
A related approach is the so-called optimal partial transport. It was initially proposed in the computer vision literature to perform image retrieval \cite{rubner1997earth,pele2008linear}, while its mathematical properties are analyzed in detail by \cite{caffarelli2010free,figalli2010optimal}. 
%
As noted in~\cite{ChizatOTFR2015} and recalled in Section \ref{sec:ExamplesPartial}, optimal partial transport is tightly linked to the generalized transport proposed in~\cite{piccoli2014generalized,piccoli2013properties} which allows a dynamic formulation of the optimal partial transport problem.
%
The contributions in \cite{piccoli2014generalized} were inspired by \cite{benamou2003numerical} where it is proposed to relax the marginal constraints and to add an $L^2$ penalization term instead.
%
%On a numerical aspect, while dynamic formulations of optimal transport (and generalizations) are useful for low-dimensional problems where the computational domain can be uniformly discretized, they do not scale to higher dimensions. In sharp contrast, the celebrated ``static'' formulation by Kantorovich~\cite{Kantorovich42} of optimal transport as a linear program is able to cope with discrete measures (i.e.\ sums of Diracs) in arbitrary dimension, with a complexity which scales only with the number of Diracs.
%%
\paragraph{Wasserstein-Fisher-Rao metric and relation with recent work.}

A new metric between measures of non equal masses has recently and independently been proposed by~\cite{ChizatOTFR2015,new2015kondratyev}. This new metric interpolates between the Wasserstein $W_2$ and the Fisher-Rao (also known as Hellinger) metrics. It is defined through a dynamic formulation, corresponding formally to a Riemannian metric on the space of measures, which generalizes the formulation of optimal transport due to Benamou and Brenier~\cite{benamou2000computational}. 

% This metric has also been introduced at the same time in~\cite{new2015kondratyev}, where they study associated topological properties,  gradient flows and Riemannian calculus on the space of measures.

\iffalse % % BEGIN COMMENT %%%%%%%%%%%%%
\todo{Gabriel: I think the following paragraph could be removed.}

Let us introduce this Wasserstein-Fisher-Rao metric, denoted by $\WF$, from a physical point of view and in a smooth setting. Let $\Omega$ be a convex domain in $\R^d$ and $\rho_0,\rho_1$ two smooth and positive functions of finite integrals. The distance between $\rho_0$ and $\rho_1$ is given by the minimization over $v(t,x) \in \R^d$ and a time dependent vector field and $g(t,x)$ a real valued function of
\begin{equation}\label{WF}
\frac12 \int_0^1 \left[ \int_{\Omega} |v(t,x)|^2 \rho(t,x) \d x  + \delta^2 \int_{\Omega} |\alpha(t,x)|^2 \rho(t,x) \d x \right] \d t
\end{equation}
under the generalized continuity constraint and the boundary constraints
\[
\partial_t \rho(t,x) + \nabla \cdot (\rho(t,x) v(t,x)) = \alpha(t,x)\rho(t,x) \quad \rho(0,\cdot) = \rho_0 , \quad  \rho(1,\cdot) = \rho_1\, .
\]
\fi % % END COMMENT %%%%%%%%%%%%%%%%%%%

In~\cite{ChizatOTFR2015}, we proved existence of geodesics, presented the limit models (for extreme values of mass creation/destruction cost) and proposed a numerical scheme based on first order proximal splitting methods. We also thoroughly treated the case of two Dirac masses which was the first step towards a Lagrangian description of the model. This metric is the prototypical example for the general framework developed in this article. It thus enjoys both a dynamic formulation and a static one (Sect.~\ref{sec:equivalence WF}). %It is also sufficiently simple so that its geometry (and in particular curvature) can be analyzed in detail, which is useful to get a deep insight about the properties of our generic class of metrics. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Contribution}
\label{sec:IntroContribution}
The initial motivation of this article is studying of the  Wasserstein-Fisher-Rao ($\WF$) metric. For two non-negative densities $\rho_0$, $\rho_1$ on a domain $\Omega \subset \R^d$ it is informally obtained as
\begin{align}
	\label{eq:WFInformal}
	\WF^2(\rho_0,\rho_1) \eqdef \inf_{(\rho,v,\alpha)} \int_0^1 \int_{\Omega} \left( \frac{1}{2} |v_t(x)|^2 + \frac{1}{2} g_t(x)^2 \right)\,\d \rho_t(x)\,\d t
\end{align}
where $(\rho_t)_{t\in [0,1]}$ is a time-dependent density that interpolates between $\rho_0$ and $\rho_1$, $(v_t)_{t\in [0,1]}$ is a velocity field that describes the movement of mass and $(g_t)_{t\in [0,1]}$ a scalar field that models local growth and destruction of mass. They must together satisfy (distributionally) the continuity equation with source
\begin{align}
	\label{eq:ContinuityEqInformal}
	\partial_t \rho_t + \nabla \cdot (\rho_t\,v_t) = \rho_t\,g_t.
\end{align}

%This article presents two sets of contributions. The first one (Section~\ref{sec:geometry}) studies in detail the geometry of the $\WF$ metric and related functionals. It is both of independent interest and serves as a motivation to introduce the second class of contributions.
%Formula \eqref{eq:WFInformal} is formally interpreted as a particular case of a family of Riemannian metrics on a semi-direct product of groups between diffeomorphisms and scalar functions. The diffeomorphisms account for mass-conservative transportation, the scalar fields act as pointwise mass multipliers.
%
%The main result of this part is the formal derivation of a submersion of this semi-direct product of groups into the space of positive measures, equipped with a metric from this family (Proposition \ref{thm:Submersion}). This corresponds to a generalization to $\WF$ of the Riemannian submersion first introduced by Otto in the optimal transport case \cite{OttoPorousMedium}. 
%
%A first application of this result is the computation of the sectional curvature of the $\WF$ space (Proposition \ref{prop-curvature}). A second application is the definition of a Monge-like formulation, i.e.\ the computation of $\WF$ in terms of a transport diffeomorphism and a pointwise mass multiplier (Section~\ref{Monge}).

In Section \ref{sec:dynamic}, we generalize this model and look at a wider family of dynamic problems given by
\begin{align}
	\label{eq:DynamicInformal}
	C_D(\rho_0,\rho_1) = \inf_{(\rho,v,\alpha)} \int_0^1 \int_{\Omega} f\big(x,\rho_t(x),v_t(x) \cdot \rho_t(x), g_t(x) \cdot \rho_t(x) \big)\,\d x\,\d t
\end{align}
where the infimum is again taken over solutions of \eqref{eq:ContinuityEqInformal}. Here, for $(\rho,v,g)\in \R_+\times \R^d\times \R$, $f(x,\rho,v \cdot \rho, g \cdot \rho)$ gives the \emph{infinitesimal cost} of moving  a particle of mass $\rho$ at $x$ in direction $v$ while undergoing an infinitesimal scaling by the (signed) rate of growth $g$.
%
Note that in the two last arguments of $f$ we multiply $v$ and $\alpha$ by $\rho$. This corresponds to the velocity to momentum change of variables proposed in \cite{benamou2000computational} to obtain a convex problem. We show that this problem admits a dual formulation (Proposition~\ref{prop: dynamic dual}) and allows to define geodesic metrics on the space of nonnegative measures (Proposition~\ref{prop:metricproperty}).

Our main goal in this article is to propose a Kantorovich-like formulation for this family of problems, where the time variable is removed. This requires to adapt the definitions as done in Section~\ref{sec : general static problem}.  We introduce a new Kantorovich-like class of \emph{static} problems of the form
\begin{align}
	\label{eq:StaticInformal}
	C_K(\rho_0,\rho_1) = \inf_{(\gamma_0,\gamma_1)} \int_{\Omega \times \Omega} c(x,\gamma_0(x,y),y,\gamma_1(x,y))\,\d x\,\d y
\end{align}
where $(\gamma_0,\gamma_1)$ are two \emph{semi-couplings} between $\rho_0$ and $\rho_1$, describing analogously to standard optimal transport, how much mass is transported between any pair $x$, $y \in \Omega$. Two semi-couplings are required, to be able to describe changes of mass during transport. The function $c(x_0,m_0,x_1,m_1)$ determines the cost of transporting a quantity of mass $m_0$ from $x_0$ to a (possibly different) quantity $m_1$ at $x_1$.
It is a crucial assumption of our approach that $c(x,\cdot,y,\cdot)$ is jointly positively 1-homogeneous and convex in the two mass arguments. This ensures that \eqref{eq:StaticInformal} can be rigorously defined as an optimization problem over measures and that the resulting problem is convex.
A dual problem is established (Proposition \ref{prop: duality}).
Analogous to standard optimal transport, when $c$ induces a metric over pairs of location and mass, then \eqref{eq:StaticInformal} defines a metric over the space of nonnegative measures (Theorem \ref{th:metric}).

In Section \ref{sec:DynamicToStatic}, under suitable assumptions on $f$, we establish equivalence between \eqref{eq:StaticInformal} and \eqref{eq:DynamicInformal} when $c$ is chosen to be the \emph{minimal path} cost induced by $f$ (Theorem \ref{th: continuous static general} and Proposition \ref{prop : alternative dynamic/static}). This is our main result, which is analogous to the Benamou-Brenier formula for classical optimal transport.

Finally, we apply those results to two unbalanced optimal transport models. 
Section \ref{sec:ExamplesPartial} introduces a dynamic formulation and gives duality results for a family of metrics obtained from the optimal partial transport problem. This is reminiscent of --- and generalizes --- the results in \cite{piccoli2013properties,piccoli2014generalized}.
The case of the $\WF$ metric is treated in Section \ref{sec:equivalence WF}. In Section \ref{sec:StaticGamma}, it is shown how standard static optimal transport is obtained as a limit (in the sense of $\Gamma$-convergence) of the $\WF$ metric, thus complementing a previous result of~\cite{ChizatOTFR2015} obtained for dynamic formulations. 

%While being motivated by Section \ref{sec:geometry}, Sections \ref{sec : general static problem} to \ref{sec:Examples} are mathematically self-contained. Readers not familiar with infinite dimensional Riemannian geometry do therefore not necessarily need to read Section \ref{sec:geometry} before proceeding to the rest of the paper.

%
%This article presents two sets of contributions. The first one (Section~\ref{sec:geometry}) studies in detail the geometry of the Wasserstein-Fisher-Rao ($\WF$) metric. It is both of independent interest and serves as the main motivation to introduce the second class of contributions. 
%%
%The main contribution of this first part is the formal derivation in Proposition \ref{Submersion} of a submersion from a semi-direct product of groups with a flat metric to the space of positive measures endowed with the $\WF$ metric. These groups are diffeomorphisms to account for mass transportation and positive functions acting as pointwise mass multipliers. 
%%
%This corresponds to a generalization to $\WF$ of the Riemannian submersion first introduced by Otto in~\cite{OttoPorousMedium} in the optimal transport case. 
%%
%A first application of this result is the computation of the sectional curvature of the $\WF$ space in Proposition \ref{thm:Curvature}. A second application is the definition in Section~\ref{Monge} of a ``Monge'' formulation, i.e.\ the computation of $\WF$ in terms of a transport diffeomorphism and a pointwise mass multiplier.
%
%
%The second set of contributions introduces and studies a general class of unbalanced optimal transport metrics, which enjoy both a static and a dynamic formulation. 
%%
%We introduce in Section~\ref{sec : general static problem} a new Kantorovich formulation and its dual (\thref{th: duality}) which can be seen as a generalization of standard optimal transport. It defines a metric over positive measures if the ground cost is a metric over position and mass (\thref{th:metric}). Under suitable assumptions the resulting metric is weakly* continuous (\thref{th : continuity continuous static}).
%%
%Then, in Section~\ref{sec:DynamicToStatic} a dynamic formulation and its dual (\thref{th: dynamic dual}) are introduced. The metric defined through these dynamic problems can also be computed by our static formulation, when one sets the ground cost to be equal to the metric between Diracs (\thref{th: continuous static general,cor : alternative dynamic/static}). 
%%
%Finally, in Section~\ref{sec:Examples}, we apply those results to two unbalanced optimal transport models. \thref{th:POT dyn/stat} introduces a dynamic formulation and gives duality results for a family of metrics obtained from the partial optimal transport problem. This is reminiscent of---and generalizes---the results in \cite{piccoli2013properties,piccoli2014generalized}. Our approach also applies to the $\WF$ metric, which can thus be computed through a static formulation (\thref{th: continuous static}). \thref{th:static gamma convergence} shows how standard static optimal transport is obtained as a limit (in the sense of $\Gamma$-convergence) of the $\WF$ metric, thus complementing a previous result of~\cite{ChizatOTFR2015} obtained for dynamic formulations. 



%%%%%%%%%%%%%%
\subsection[Relation with Liero,Mielke,Savare 2015]{Relation with \cite{LieroMielkeSavareLong,LieroMielkeSavareShort}}

After completing this paper, we became aware of the independent work of \cite{LieroMielkeSavareLong,LieroMielkeSavareShort}. In these two papers the authors develop and study a similar class of ``static'' transportation-like problems as here. This huge body of work contains many theoretical aspects that we do not cover. For instance measures defined over more general metric spaces are considered, while we work over $\R^d$.
%
The construction of~\cite{LieroMielkeSavareLong} defines three equivalent static formulations. Their third ``homogeneous'' formulation is closely related (by a change of variables) to our ``semi-couplings'' formulation. Their first formulation gives an intuitive and nice interpretation of this class of convex programs as a modification of the original optimal transportation problem where one replaces the hard marginal constraints by soft penalization using  Csisz\'ar $f$-divergences. The dual of this first formulation is related to the dual of our formulation by a logarithmic change of variables, see Corollary \ref{cor : static log-entropic}. Quite interestingly, the same idea is used in an informal and heuristic way by~\cite{FrognerNIPS} for applications in machine learning, where soft marginal constraints is the key to stabilize numerical results. 
%
The authors of~\cite{LieroMielkeSavareLong,LieroMielkeSavareShort} study dynamical formulations in the Wasserstein-Fisher-Rao setting (that they call the ``Hellinger-Kantorovich'' problem). This allows them to make a detailed analysis of the geodesic structure of this space. In contrast, we study a more general class of dynamical problems, but restrict our attention to the equivalence with the static problem. Another original contribution of our work is the proof of the metric structure (in particular the triangular inequality) for static and dynamic formulations when the underlying cost over the cone manifold $\Omega \times \R^+$ is related to a distance. 
% 
%Lastly, our geometric study of Section \ref{sec:geometry}, and in particular the Riemannian submersion structure, the explicit sectional curvature computation and the Monge problem appear to be original contributions. Note that along these lines, the work of~\cite{LieroMielkeSavareLong} proves a lower bound on the Alexandrov curvature in the $\WF$ case, which in particular allows these authors to state sufficient condition for the $\WF$ space to have positive curvature. In a smooth setting, we find similar results in Proposition \ref{prop-curvature} and Corollary \ref{th:CorollaryCurvature}.

%%%%%%%%%%%%%%
\subsection{Preliminaries and notation}
We denote by $C(X)$ the Banach space of real valued continuous functions on a compact set $X\subset \R^d$ endowed with the sup norm topology. Its topological dual is identified with the set of Radon measures, denoted by $\mathcal{M}(X)$ and the dual norm on $\mathcal{M}(X)$ is the total variation, denoted by $|\cdot|_{TV}$. Another useful topology on $\mathcal{M}(X)$ is the weak* topology arising from this duality: a sequence of measures $(\mu_n)_{n\in \N}$ weak* converges towards $\mu \in \mathcal{M}(X)$ if and only if for all $u \in C(X)$, $\lim_{n\rightarrow + \infty}\int_{X} u \, \d\mu_n = \int_{X} u \,\d\mu$. According to that topology, $C(X)$ and $\mathcal{M}(X)$ are topologically paired spaces (the elements of each space can be identified with the continuous linear forms on the other), this is a standard setting in convex analysis.
%Any bounded subset of $\mathcal{M}(X)$ (for the total variation) is relatively sequentially compact for the weak* topology.
We also use the following notations:
\begin{itemize}
	\item $\mathcal{M}(X)$ is the vector space of Radon measures and $\mathcal{M}_+(X)$ the cone of \emph{nonnegative} Radon measures;
	%\item For $M$ a given manifold, $TM$ denotes the tangent bundle of $M$ and $T_pM$ the tangent space at a point $p \in M$.
	%\item $\Dens(X)$ the set of finite Radon measures that have smooth positive density w.r.t.\ a reference volume form $\nu$;

	\item $\mu \ll \nu$ means that the $\R^m$-valued measure $\mu$ is absolutely continuous w.r.t.\ the positive measure $\nu$. We denote by $\dens{\mu}{\nu} \in (L^1(X,\nu))^m$ the density of $\mu$ with respect to $\nu$;

	\item Ffr a (possibly vector) measure $\mu$, $|\mu| \in \mathcal{M}_+(X)$ is its variation;

	%\item for a positively homogeneous function $f$, we denote by $f(\mu)$ the measure defined by $f(\mu)(A) \eqdef \int_A f(\d\mu/\d\lambda) \d\lambda$ for any measurable set $A$, with $\lambda$ satisfying $|\mu| \ll \lambda$. The homogeneity assumption guarantees that this definition does not depend on $\lambda$;
	%\item For a map $\varphi: M \mapsto N$ between two manifolds $M,N$, $T\varphi$ denotes the tangent map of $\varphi$. For a given Riemannian metric $g$ on $N$, the pull-back of $g$ by $\varphi$ is denoted by $\varphi^*g$ and defined by $(\varphi^*g)(x)(v_x,v_x) \eqdef g(\varphi(x))(T_x\varphi(v_x),T_x\varphi(v_x))$.
	\item $\pfwd{T} \mu$ is the image measure of $\mu$ through the measurable map $T: X_1 \to X_2$, also called the pushforward measure. It is given by $\pfwd{T} \mu (A_2) \eqdef \mu(T^{-1}(A_2))$;
	% When $X_1= X_2$ is a manifold and $T$ is a diffeomorphism, we denote $\pfwd{T}$ by $\pfwdM{T}$.

	\item $\delta_x$ is a Dirac measure of mass $1$ located at the point $x$;

	\item $\iota_{\mathcal{C}}$ is the (convex) indicator function of a convex set $\mathcal{C}$ which takes the value $0$ on $\mathcal{C}$ and $+\infty$ everywhere else;

	\item if $(E,E')$ are topologically paired spaces and $f : E \to \R \cup \{+ \infty\}$ is a convex function, $f^*$ is its Legendre transform i.e.\ for $y \in E'$, $f^*(y) \eqdef \sup_{x\in E} \langle x, y \rangle - f(x) $; %The subdifferential of $f$ is denoted $\D f$ and is the set valued map $x \mapsto \{ y\in E' : \forall x' \in E, \, f(x')-f(x) \geq \langle y, x'-x \rangle \}$.

	\item for $n \in \N$ and a tuple of distinct indices $(i_1,\ldots,i_k)$, $i_l \in \{0,\ldots,n-1\}$ the map
\begin{equation}
	\Proj_{i_1,\ldots,i_k} : \Omega^n \rightarrow \Omega^k
\end{equation}
denotes the canonical projection from $\Omega^n$ onto the factors given by the tuple $(i_1,\ldots,i_k)$;

%Finally, when $\mu$ is a measure on $[0,1] \times \Om$ which time marginal is absolutely continuous with respect to the Lebesgue measure on $[0,1]$, we denote by $(\mu_t)_{t\in[0,1]}$ the ($\d t$-a.e.\ uniquely determined) family of measures satisfying $\mu = \int_0^1 (\mu_t \otimes \delta_t ) \d t$, where $\otimes$ denotes the product of measures. This is a consequence of the disintegration theorem (see for instance ~\cite[Theorem 5.3.1]{ambrosio2006gradient}) which we frequently use without explicitly mentioning it. In order to alleviate notations, we replace the integral expression of $\mu$ by $\mu = \mu_t \otimes \d t$.
%

	\item the truncated cosine is defined by $\trucos : z \mapsto \cos(|z|\wedge \frac{\pi}{2})$;
	\item we denote by $f\wedge g$ the biggest function (or measure) that is smaller than both $f$ and $g$. This is to be contrasted with the notation $\min S$ which for a totally ordered set $S$ denotes its smallest element.
	%\todo{len:define the minimum of 2 functions/two measures}
\end{itemize}






==> Submission Final JFA/Static.tex <==
% !TEX root = ../DynamicToStatic.tex

%%%%%%%%%%%%%%%%%%%%%%%%%
%STATIC PROBLEM
%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Static Kantorovich Formulations}
\label{sec : general static problem}
The classical Kantorovich formulation of optimal transport, for two probability measures $\mu,\nu$ on a set $X$ and with a transport cost $c:(x,y)\mapsto \R \cup \{\infty\}$, is
\[
\inf \left\{ \int_{X^2} c(x,y) \d \gamma(x,y)\;;\; \gamma \in \mathcal{M}_+(X^2), (\Proj_0)_\# \gamma = \mu \text{ and } (\Proj_1)_\# \gamma = \nu \right\}.
\]
A nonnegative measure on $X^2$ that satisfies the marginal constraints is called a \emph{coupling} of $\mu$ and $\nu$. If now $\mu$ and $\nu$ have different total masses, two issues arise: (i) the set of couplings between $\mu$ and $\nu$ is empty and (ii) the cost needs also to describe the effort necessary to make the mass vary. We propose in this section a generalized Kantorovich problem that is valid for arbitrary nonnegative measures. %It is introduced in Definition \ref{def:extended kantorovich} and its dual formulation in Theorem \ref{th: duality}. When This Kantorovich formulation does not need the cost on the product space to be related to a distance, yet, when it is the case and under mild assumptions described below, the Kantorovich formulation defines a distance on $\mathcal{M}_+(X)$ as shown in Theorem \ref{th:metric}.l

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Definitions}
In what follows, $\Omega \subset \R^d$ is a compact set, $x$ typically refers to a point in $X$ and $m$ to a mass.  We first define a cost function, which takes as input not only two points in space but also two masses: it can be though of as the cost of matching two Dirac measures of arbitrary mass.

\begin{definition}[Cost function]
	\label{def:CostFunction}
	In the sequel, a \emph{cost function} is a function 
	\[
		c : 
		\begin{array}{lcl}
			(\Omega \times [0, + \infty[) ^2 &\to & [0,+ \infty] \\
			(x_0,m_0),(x_1,m_1) &\mapsto &c(x_0,m_0,x_1,m_1)
		\end{array}
	\]
which is l.s.c.\ in all its arguments and jointly sublinear in $(m_0, m_1)$. It is implicitly defined as $+\infty$ outside of its domain of definition.
\end{definition}

A \emph{sublinear} function is by definition a positively 1-homogeneous and subadditive function, or equivalently, a positively 1-homogeneous and convex function. The joint subadditivity of $c$ in $(m_0,m_1)$ guarantees that it is always better to send mass from one point to another in one single chunk. This sublinearity requirement can be interpreted as the generalization of the fact that, in classical optimal transport, the cost of moving mass is linear with the mass.

In order to allow for variations of mass, we need to adapt the constraint set of standard optimal transport by introducing the notion of \emph{semi-couplings}. These are relaxed couplings with only one marginal being fixed. 

\begin{definition}[Semi-couplings]
For two marginals $\rho_0, \rho_1 \in \mathcal{M}_+(\Omega)$, the set of semi-couplings is
	\begin{align}
		\Gamma(\rho_0,\rho_1) \eqdef \left\{
			(\gamma_0,\gamma_1) \in \big(\mathcal{M}_+(\Omega^2)\big)^2 \colon
			\pfwd{(\Proj_0)} \gamma_0 = \rho_0,\, \pfwd{(\Proj_1)} \gamma_1 = \rho_1
			\right\}.
	\end{align}
\end{definition}

Informally, $\gamma_0(x,y)$ represents the amount of mass that is taken from $\rho_0$ at point $x$ and is then transported to an (possibly different, to account for creation/destruction) amount of mass $\gamma_1(x,y)$ at point $y$ of $\rho_1$. These semi-couplings allow us to formulate a novel static Kantorovich formulation of unbalanced optimal transport as follows. 

\begin{definition}[Unbalanced Kantorovich problem]
	\label{def:extended kantorovich}
	For a cost function $c$ we introduce the functional
	\begin{align}
		J_K(\gamma_0,\gamma_1) \eqdef \int_{\Omega^2} c \left( x,\dens{ \gamma_0}{ \gamma},y,\dens{ \gamma_1}{ \gamma}\right) \d \gamma(x,y)\, ,
	\end{align}
where $\gamma \in \mathcal{M}_+(\Omega^2)$ is any measure such that $\gamma_0, \gamma_1 \ll \gamma$. This functional is well-defined since $c$ is jointly 1-homogeneous w.r.t.\ the mass variables (see Definition \ref{def:CostFunction}).
	The corresponding optimization problem is
	\begin{align}
	\label{eq: static problem}
	%\tag{Q_{\mathcal{M}}}
		C_K(\rho_0,\rho_1)  \eqdef \inf_{(\gamma_0,\gamma_1) \in \Gamma(\rho_0,\rho_1)}
			J_K(\gamma_0,\gamma_1)\,.
	\end{align}
\end{definition}


\begin{proposition}
	\label{prop:KMinimizers}
	If $c$ is a \emph{cost function} then a minimizer for $C_K(\rho_0,\rho_1)$ exists.
\end{proposition}
\begin{proof}
By Lemma~\ref{lem:dualitymeasures}, $J_K$ is weakly* l.s.c.\ on $\mathcal{M}(\Omega^2)$. Since $\Omega$ is compact and the marginals $\rho_0,\rho_1$ have finite mass, $\Gamma(\rho_0,\rho_1)$ is tight and thus weakly* pre-compact. It is also closed so $\Gamma(\rho_0,\rho_1)$ is weakly* compact and any minimizing sequence admits a cluster point which is a minimizer (the minimum is not assumed to be finite).
\end{proof}

\begin{example}
\label{ex : example cost static}
	Standard optimal transport problems with a nonnegative, l.s.c.\ cost $\tilde{c}$ are retrieved as particular cases, by taking 
	\begin{align*}
		c(x_0,m_0,x_1,m_1) & = 
		\begin{cases}
			m_0 \cdot \tilde{c}(x,y)& \text{if } m_0 = m_1\,, \\
			+ \infty & \text{otherwise.}
		\end{cases}
	\end{align*}
	\end{example}

This example shows that, unlike the dynamic problems of the previous section, these \emph{semi-coupling} formulations form a proper generalization of the Kantorovich problems. In particular, the properties that we prove next (duality, metric) can be particularized to recover well-known properties of classical optimal transport. Other examples, in particular the $\WF$-metric, are studied in more detail in Section \ref{sec:Examples}.

%\begin{example}
%	The interpolation between optimal transport and the Fisher-Rao metric is obtained \todo{at this stage, isn't it to early to state this? Otherwise, explain what ``obtained'' means}  by choosing the cost function \eqref{eq:GeneralizedCost:OTFR}.In this case, the optimization problem~\eqref{eq: static problem} is a conic program involving quadratic cones, and if the measures $(\rho_0,\rho_1)$ are finite sums of Diracs, it can be solved using interior point solvers~\cite{nesterov1994interior}. 
%\end{example}

%\begin{example}
%One can recover the ``flat metric'' (a metric between total variation and $W_1$, see the definition of $W^{1,1}_1$ in \cite{piccoli2013properties}), by taking
%	\begin{align*}
%		c(x_0,m_0,x_1,m_1) & = 
%		\begin{cases}
%			|x_0-x_1|\min (m_0,m_1) + |m_1-m_0|& \text{if $|x_0-x_1|<2$}\,, \\
%			m_0 + m_1 & \text{otherwise.}
%		\end{cases}
%	\end{align*}
%\end{example}
%
%More examples will be studied with more details in the last section of this article.

%%%%%%%%%%%%%%%%%%%%%%%%%
% PROPERTIES
%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Properties of semi-coupling problems}


%%%%%%% METRIC PROPERTY
A central property of optimal transport is that it can be used to lift a metric from the base space $\Omega$ to the space of probability measures over $\Omega$ (cf.\ \cite[Chapter 6]{villani2009oldnew}). We now show that this extends to the unbalanced framework. We first introduce the space $\Cone(\Omega)$, a standard construction in topology which, in our context, can be understood as the space of Dirac measures of arbitrary mass (endowed with the weak* topology).


\begin{definition}[Cone]
The space $\Cone(\Omega)$ is defined as the space $\Omega \times \R_+$ where all the points with zero mass $\Omega \times \{0\}$ are identified to one point. It is endowed with the quotient topology (note that subtleties appear in the non-compact setting, see~\cite{LieroMielkeSavareLong}).
\end{definition}
\begin{theorem}[Metric]
\label{th:metric}
Let $c$ be a cost function such that, for some $p \in [1, + \infty[$ 
\begin{align}
	\label{eq:CMetric}
	(x_0,m_0), (x_1,m_1) \mapsto c(x_0,m_0,x_1,m_1)^{1/p}
\end{align}
is a metric on  $\Cone(\Omega)$. Then $C_K^{1/p}$ defines a metric on $\mathcal{M}_+(\Omega)$.
\end{theorem}
%Remember that the space $\Cone(\Omega)$ is defined as the space $\Omega \times [0,+\infty[$ where all the points with zero mass $\Omega \times \{0\}$ collapse to one point (see Definition~\ref{def:Cone})\todo{define the cone}.
\begin{remark}
Compatibility with the cone structure implies in particular that for all $x_2\in \Omega$, $m\geq0$, 
$c(x_1, 0, x_2, m)$ must be independent of $x_1\in \Omega$ and $c(x_1,0,x_2,0)=0$.
\end{remark}
%
\begin{remark}
One can replace the word ``metric'' by ``extended metric'' (i.e.\ allowing the value $+\infty$) and the proof goes through. By considering the cost in Example \ref{ex : example cost static}, a corollary is that $C_K^{1/p}$ defines a proper metric on each equivalence class for the relation $\mu \sim \nu \Leftrightarrow \mu(\Omega) = \nu(\Omega)$. The metric property of the Wasserstein distance is thus recovered as a particular case.
\end{remark}
%%%%%%%%%%%%%%%

\begin{proof}
First, symmetry and nonnegativity are inherited from $c$. Moreover, 
\begin{multline*}
[ C_K(\gamma_0,\gamma_1) = 0 ]
\Leftrightarrow \\
[ \exists (\gamma_0, \gamma_1) \in \Gamma(\rho_0, \rho_1) : (\gamma_0= \gamma_1) \tn{ and }  (x=y \tn{ $\gamma_0$-a.e.}) ] \\
\Leftrightarrow
[ \rho_0 = \rho_1 ].
\end{multline*}
%And thus $C_K(\cdot,\cdot)^{1/p}=0$ if and only if $\rho_0=\rho_1$. 

\newcommand{\mudens}[1]{{\textstyle{\frac{#1}{\mu}}}}
\newcommand{\mudisint}[1]{{(#1|\mu)}}
It remains to show the triangle inequality. Fix $\rho_0$, $\rho_1$, $\rho_2 \in \mathcal{M}_+(\Omega)$. Take two pairs of minimizers for \eqref{eq: static problem} 
	\begin{align*}
		(\gamma_0^{01},\gamma_1^{01}) & \in \Gamma(\rho_0,\rho_1)\,, &
		(\gamma_0^{12},\gamma_1^{12}) & \in \Gamma(\rho_1,\rho_2)\,, 		
	\end{align*}
and let $\mu \in \mathcal{M}_+(\Omega)$ be such that $\pfwd{(\Proj_1)} (\gamma_0^{01},\gamma_1^{01}) \ll \mu$ and $\pfwd{(\Proj_0)} (\gamma_0^{12},\gamma_1^{12}) \ll \mu $. Denote by $\mudisint{\gamma_i^{01}}(x|y)$ the disintegration of $\gamma_i^{01}$ along the second factor w.r.t.\ $\mu$. More precisely, for all $y\in \Omega$, $\mudisint{\gamma_i^{01}}(\cdot|y)\in \mathcal{M}_+(\Omega)$ and it holds, for all $f$ measurable on $\Omega^2$, 
\begin{align*}
	\int_{\Omega^2} f\,\d\gamma_i^{01} & = \int_{\Omega} \left( \int_{\Omega} f(x,y)\,\d\mudisint{\gamma_i^{01}}(x|y) \right)\,\d\mu(y)
\end{align*}
and analogously for $\mudisint{\gamma_i^{12}}(z|y)$ along the first factor for $i=0,1$. Write $\mudens{\rho_1}(y)$ for the density of $\rho_1$ w.r.t.\ $\mu$.
%
%By an abuse of notation, we use the same letters for denoting the measures and their density w.r.t.\ $\mu$. 
We combine the optimal semi-couplings in a suitable way to define $\gamma_0$, $\gamma_1$, $\hat{\gamma} \in \mc{M}(\Omega^3)$ (via disintegration w.r.t.\ $\mu$ along the second factor):
\begin{align*}
\mudisint{\gamma_0}(x,z|y) &\eqdef
\begin{cases}
\frac{\mudisint{\gamma_0^{01}}(x|y) \otimes \mudisint{\gamma_0^{12}}(z|y)}{\mudens{\rho_1}(y)} & \tn{ if } \mudens{\rho_1}(y) >0, \\
\mudisint{\gamma_0^{01}}(x|y) \otimes \delta_{y}(z) & \tn{ otherwise, }
\end{cases} \\
\mudisint{\gamma_1}(x,z|y) &\eqdef
\begin{cases}
\frac{\mudisint{\gamma_1^{01}}(x|y) \otimes \mudisint{\gamma_1^{12}}(z|y)}{\mudens{\rho_1}(y)} & \tn{ if } \mudens{\rho_1}(y) >0, \\
\delta_{y}(x) \otimes \mudisint{\gamma_1^{12}}(z|y) & \tn{ otherwise, }
\end{cases} \\
\mudisint{\hat{\gamma}}(x,z|y) &\eqdef  
\begin{cases}
\frac{\mudisint{\gamma_1^{01}}(x|y) \otimes \mudisint{\gamma_0^{12}}(z|y)}{\mudens{\rho_1}(y)} & \tn{ if } \mudens{\rho_1}(y) >0, \\
0 & \tn{ otherwise. }
\end{cases}
\end{align*}
The interpretation of $\gamma_0$ is that all mass that leaves $x$ towards $y$, according to $\gamma_0^{01}(x,y)$, is distributed over the third factor according to $\gamma_0^{12}(y,z)$. In case the mass disappears at $y$, it is simply ``dropped'' as $\delta_y$ on the third factor. Then $\gamma_1$ is built analogously for the incoming masses and $\hat{\gamma}$ is a combination of incoming and outgoing masses.
%
For $i=0,1$ let $\gamma_i^{02} \eqdef \pfwd{(\Proj_{02})} \gamma_i$ and note that, by construction, $(\gamma_0^{02},\gamma_1^{02}) \in \Gamma(\rho_0, \rho_2)$.
In the rest of the proof, for an improved readability, when writing the functional the dummy measure $\gamma$ such that $\gamma_0, \gamma_1 \ll \gamma$ is considered as implicit and we write
	\begin{equation*}
	\label{remark : abuse of notation}
		\int_{\Omega^2} c\big(x,\gamma_0(x,y),y,\gamma_1(x,y)\big)\,\d x\,\d y
		\quad \text{for}\quad \int_{\Omega^2} c \left(x,\dens{ \gamma_0}{ \gamma},y,\dens{ \gamma_1}{ \gamma}\right) \d \gamma(x,y)\, .
	\end{equation*}
With this notation, one has
\begin{align*}
& \int_{\Omega^3} c\big(x,\gamma_0(x,y,z),y,\hat{\gamma}(x,y,z)\big) \d x\,\d y\,\d z \\
= {} & \int_{\rho(y)>0} \left( \int_{\Omega^2}
	c\big(x,\mudisint{\gamma_0^{01}}(x|y), y, \mudisint{\gamma_1^{01}}(x|y)\big)
	\frac{\mudisint{\gamma_0^{12}}(y|z)}{\mudens{\rho}(y)} \d x\,\d z \right) \d \mu(y) \\
& + \int_{\rho(y)=0} \left( \int_{\Omega^2}
	c\big(x,\mudisint{\gamma_0^{01}}(x|y),y,0\big) \delta_{y}(z) \d x\,\d z \right) \d \mu(y) \\
= {} &  \int_{\Omega} \left( \int_{\Omega}
	c\big(x,\mudisint{\gamma_0^{01}}(x|y), y, \mudisint{\gamma_1^{01}}(x|y)\big)
	\d x \right) \d\mu(y) \\
= {} & J_K(\gamma_0^{01},\gamma_1^{01}) = C_K(\rho_0,\rho_1)\, ,
\end{align*}
and analogously
\begin{align*}
	\int_{\Omega^3} c\big(y,\hat{\gamma}(x,y,z),z,\gamma_1(x,y,z)\big) \d x\,\d y\,\d z & =
	C_K(\rho_1,\rho_2)\,.
\end{align*}
%%
One finally obtains
	\begin{align*}
		 C_K(\rho_0,\rho_2)^{\frac{1}{p}} 
		 \leq {} & \Big(\int_{\Omega^2} c\big(x,\gamma_0^{02}(x,z),z,\gamma_1^{02}(x,z) \big) \d x\,\d z \Big)^{\frac{1}{p}} \\
		\overset{(1)}{\leq} {} & \Big( \int_{\Omega^3} c\big( x, \gamma_0(x,y,z),z, \gamma_1(x,y,z) \big) \d x\,\d y\,\d z \Big)^{\frac{1}{p}} \\
		\overset{(2)}{\leq} {} & 
			\Big( \int_{\Omega^3} 
			\Big[ 
			c\big( x, \gamma_0(x,y,z), y, \hat{\gamma}(x,y,z) \big)^{\frac{1}{p}} + \\
			&\qquad\qquad c\big( y, \hat{\gamma}(x,y,z), z, \gamma_1(x,y,z) \big)^{\frac{1}{p}}
			\Big]^p \d x\,\d y\,\d z 
			\Big)^{\frac{1}{p}} \\
		\overset{(3}{\leq} {} & 
			\Big( \int_{\Omega^3} c\big( x, \gamma_0(x,y,z),y, \hat{\gamma}(x,y,z)\big) \d x\,\d y\,\d z \Big)^{\frac{1}{p}} + \\
			&\qquad\qquad  \Big( \int_{\Omega^3} c\big( y, \hat{\gamma}(x,y,z), z,\gamma_1(x,y,z) \big) \d x\,\d y\,\d z\Big)^{\frac{1}{p}} \\
		\overset{(4)}{=} {} & C_K\left(\rho_0, \rho_1\right)^{\frac{1}{p}} + 
			C_K\left(\rho_1, \rho_2\right)^{\frac{1}{p}} 
		\end{align*}
	where we used (1) the convexity of $c$, (2) the fact that $c^{1/p}$ satisfies the triangle inequality, (3) Minkowski's inequality and (4) comes from the computations above. Thus $C_K(\cdot,\cdot)^{1/p}$ satisfies the triangle inequality, and is a metric. 
\end{proof}

\iffalse
%%%%% CONTINUITY

Next, we establish under reasonable assumptions on the cost $c$ that the corresponding unbalanced transport cost $C_K$ is weakly* continuous w.r.t.\ the marginals.
This is important for numerical applications, since it implies robustness when one approximates the original measures with discrete sums of Diracs. It is also crucial to study the well posedness of variational problems involving these metrics, such as for instance the definition of barycenters (see~\cite{Carlier_wasserstein_barycenter} for the classical optimal transport case). 
%
%Moreover it is a useful tool in our further analysis (Theorem \ref{th: continuous static general}).
\todo{I'd be in favor of removing this result (it is not used in the following and does not really match the flow of the article)}
\begin{theorem}[weak convergence]\label{th : continuity continuous static}
Assume that $(x,y)\mapsto c(x,1,y,1)$ tends to $0$ as $|y-x|\to 0$ and that there exists $\alpha>0$ such that $c(x,1,x,0)+c(x,0,x,1)< \alpha$ for all $x\in \Omega$, then
$
(\mu_n \rightharpoonup^* \mu) \Rightarrow (C_K(\mu_n,\mu)\to 0).
$
\end{theorem}
\begin{proof}
First, notice that the continuity near the diagonal (and thus uniform continuity by compactenss of $X$) of $c(\cdot,1,\cdot,1)$, for all $\epsilon>0$, there exists $\eta>0$ such that $|y-x|<\eta$ implies $c(x,1,y,1)<\epsilon$. In order to prove continuity the result, we choose a finite partition $(W_i)_{i\in I}$ of $\Omega$ of diameter smaller than $\eta$ such that $\mu (\partial W_i)=0$ for all $i\in I$ (the fact that this partition exists is generally known as the mosaic lemma). Since $(\mu_n)$ weakly* converges to $\mu$, one has, by the Portmanteau lemma, that $\mu_n(W_i) \to \mu(W_i)$ for all $i\in I$. Let us build a pair of semi-couplings $(\gamma_0^{(n)},\gamma_1^{(n)})$ for all $n\in \mathbb{N}$ as follows.

First, $\gamma_0^{(n)}|_{W_i\times W_j}=\gamma_1^{(n)}|_{W_i\times W_j}=0$ if $i\neq j$ or if $\mu_n(W_i)=\mu(W_j)=0$. Otherwise, if $\mu_n(W_i)>\mu(W_i)$ define
\[
\left\{
\begin{aligned}
\gamma_0^{(n)}|_{W_i\times W_i}&=(\mu_n|_{W_i} \otimes \mu|_{W_i})/\mu_n(W_i) + (1-\mu(W_i)/\mu_n(W_i))\, \mathrm{diag}_\# \mu_n\\
\gamma_1^{(n)}|_{W_i\times W_i}&=(\mu_n|_{W_i} \otimes \mu|_{W_i})/\mu_n(W_i).
\end{aligned}
\right.
\]
where $\mathrm{diag}(x)=(x,x)$ maps $\Omega$ to the diagonal of $\Omega^2$. If $\mu(W_i)\geq \mu_n(W_i)$ use the same definition but with the role of $\mu$ and $\mu_n$ exchanged. 
%
By construction, $\gamma_0^{(n)}$ and $\gamma_1^{(n)}$ satisfy the semi-coupling constraint and one can now control $C_K(\mu_n,\mu)$ as follows:
\begin{align*}
C_K(\mu_n,\mu) \leq J_K(\gamma_0^{(n)},\gamma_1^{(n)})
\leq \sum_{i\in I} \epsilon \max(\mu_n(W_i),\mu(W_i)) + \alpha \vert \mu_n(W_i)-\mu(W_i)\vert
\end{align*}
and the last term tends to $\epsilon \mu(\Omega)$ as $n\to \infty$. Since $\epsilon>0$ is arbitrary, it follows that $C_K(\mu_n,\mu)\to 0$.
\end{proof}
\fi
%\begin{theorem}
%\label{th : continuity continuous static}
%Assume that $c$ satisfies the assumptions of \thref{th:metric} for some $p\in [1, + \infty[$, and moreover that
%\begin{enumerate}[{(A}1{)}]
%	\item $c(\cdot, 1, \cdot,0)$ is bounded; \label{continuity asp 1}
%	\item the family of functions $(c_{x,x})_{x\in \Omega} \eqdef (c(x,\cdot, x, \cdot))$ is uniformly continuous at $(m_0,m_1)=(1,1)$; \label{continuity asp 2}
%	\item there exists $(q,\alpha) \in ]0,\infty[^2$ such that, $\forall (x,y)\in \Omega^2$, $c(x,1,y,1) \leq \alpha |x-y|^q$.\label{continuity asp 3}
%\end{enumerate}
%Then $C_K$ is continuous for the weak* topology on $\mathcal{M}_+(\Omega)^2$.
%\end{theorem}
%
%\begin{remark}
%	Let us briefly comment on the assumptions on the cost function.
%	\begin{itemize}
%		\item (A\ref{continuity asp 1}) provides that mass for which no assignment partner can be found can be removed with a finite cost.
%		\item (A\ref{continuity asp 2}) guarantees that small deviations in mass only inflict a small additional matching cost. Note that this assumption is not met by classical optimal transport.
%		\item (A\ref{continuity asp 3}) states that as long as the initial and final mass are the same, the extended transport cost is always bounded from above by the classical optimal transport cost. For example, the cost between two Diracs $\delta_{x}$ and $\delta_{y}$ is bounded by $\alpha\,|x-y|^q$.
%	\end{itemize}
%\end{remark}
\iffalse
\begin{theorem}
	\label{th : continuity continuous static}
	Assume $c$ satisfies the assumptions of Theorem \ref{th:metric} and:
	\begin{enumerate}[{(A}1{)}]
		\item Continuity of the spatial metric: $(x,y) \mapsto c(x,1,y,1)$ is continuous. \label{asp:ContinuityContinuity}
		\item Finite cost of mass removal: there exists $x \in \Omega$ such that $c(x,1,x,0) < +\infty$. \label{asp:ContinuityFiniteness}
	\end{enumerate}
	Then $C_K$ is continuous for the weak* topology on $\mc{M}_+(\Omega)^2$.
\end{theorem}
%
\begin{lemma}
	\label{lemma: continuity aux lemma}
	Under the assumptions of Theorem \ref{th : continuity continuous static}, for some $p\in [1,+\infty[$,
	\begin{enumerate}[{(B}1{)}]
		\item $(x_0,x_1) \mapsto c(x_0,1,x_1,1)^{1/p}$ is equivalent to the Euclidean metric; \label{asp:ContinuityInterEquivalence}
		\item $x \mapsto c(x,1,x,0)$ is bounded on $\Omega$;
		\label{asp:ContinuityInterBounded}
		\item the family of functions $\{m \mapsto c(x,1,x,m)\}_{x \in \Omega}$ is  equicontinuous at $m=1$. \label{asp:ContinuityInterContinuity}
	\end{enumerate}
\end{lemma}
\begin{proof} \textit{(B\ref{asp:ContinuityInterEquivalence}):}
	Two metrics $d_1$, $d_2$ are equivalent when
	\begin{align*}
		d_1(x_n,x) \rightarrow 0 \Leftrightarrow d_2(x_n,x) \rightarrow 0\,.
	\end{align*}
	Let $d_1(x,y) = |x-y|$ the Euclidean metric on $\Omega$ and $d_2(x,y) = c(x,1,y,1)^{1/p}$. Assumption (A\ref{asp:ContinuityContinuity}) implies ``$\Rightarrow$''.
	Now we want to show that $d_2(x_n,x) \rightarrow 0$ implies $d_1(x_n,x) \rightarrow 0$. Let $\veps > 0$ and let $S = \Omega \cap B(x,\veps)$ ($B(x,\veps)$ denoting the open ball of radius $\veps$ around $x$). Then $\Omega \setminus S$ is compact. Therefore $x' \mapsto d_2(x,x')$ attains its minimum $\delta$ over $\Omega \setminus S$ on that set and by the metric property $\delta > 0$. Since $d_2(x_n,x) \rightarrow 0$ there is some $N \in \mathbb{N}$ such that $d_2(x_n,x) < \delta$ for $n>N$ and consequently $x_n \in B(x,\veps)$ for $n>N$.
	
	\textit{(B\ref{asp:ContinuityInterBounded})} For any $y \in \Omega$ one has by the triangle inequality and the identification of zero-mass points $c(y,1,y,0)^{1/p} \leq c(y,1,x,1)^{1/p} + c(x,1,x,0)^{1/p}$. The first term is bounded since it is continuous in $y$ and $\Omega$ is compact. The second term is bounded by assumption (A\ref{asp:ContinuityFiniteness}).
	
	\textit{(B\ref{asp:ContinuityInterContinuity})} Let $C$ be the uniform bound of $c(x,1,x,0)$ over $\Omega$. By 1-homogeneity and triangle inequality it holds $c(x,1,x,2) \leq \big( c(x,1,x,0)^{1/p} + c(x,2,x,0)^{1/p} \big)^p \leq C\,\big( 1+ 2^{1/p} \big)^p \eqdef C'$. By convexity of $c$, $c(x,m,x,1) \leq |m-1|\,C'$ for $m \in [0,2]$. As $c$ is nonnegative, the family $\{m \mapsto c(x,1,x,m) \}_{x \in \Omega}$ is therefore uniformly continuous at $m=1$.
\end{proof}

\begin{proof}[Proof of Theorem \ref{th : continuity continuous static}]
Throughout this proof we are going to use the properties (B\ref{asp:ContinuityInterEquivalence}) to (B\ref{asp:ContinuityInterContinuity}) established in Lemma \ref{lemma: continuity aux lemma}.
Thanks to the triangle inequality, we only need to check that, if $\rho_n \rightharpoonup^* \rho$ then $C_K(\rho_n,\rho) \allowbreak \to 0$.

Recall that weak* convergence implies (1) convergence of the total masses and (2) convergence for the $p$-Wasserstein distance $W_p$ ($p\in [1,+\infty[$) of the rescaled measures (see for instance \cite[Theorem 7.12]{cedric2003topics}). We denote by $W_{p,c}$ the Wasserstein metric induced by the ground metric $(x,y) \mapsto c(x,1,y,1)^{1/p}$. By property (B\ref{asp:ContinuityInterEquivalence}) this ground metric induces the same topology on $\Omega$ as the Euclidean metric. Therefore both metrics induce the same space of continuous functions $C(\Omega)$ and therefore convergence of $W_p$ and $W_{p,c}$ is equivalent, too.\todo{check argument (reviwer2)}

If $\rho = 0$ then, by taking $(\gamma_n \eqdef \pfwd{(\id,\id)} \rho_n, 0) \in \Gamma(\rho_n, \rho)$ we see that, by property (B\ref{asp:ContinuityInterBounded}),
\[
C_K(\rho_n, \rho) \leq \int_{\Omega^2} c(x_0,1,x_1,0)\, \d \gamma_n(x_0,x_1) \leq (\sup_{x \in \Omega} |c(x,1, x,0) |) \cdot \rho_n(\Omega) \to 0 \, .
\]
Otherwise, let us assume that for all $n\in \mathbb{N}$, $\rho_n(\Omega)>0$ as it is eventually true. Introduce $\mnorm(\rho_n) \eqdef (\rho(\Omega)/\rho_n(\Omega)) \cdot \rho_n$. It holds, by the triangle inequality,
\[
C_K^\frac1p (\rho_n,\rho) \leq C_K^\frac1p (\rho_n,\mnorm(\rho_n)) + C_K^\frac1p (\mnorm(\rho_n),\rho)\, .
\]
On the one hand, by choosing $\gamma_0 = \pfwd{(\id,\id)} \rho_n$ and  $\gamma_1 = (\rho(\Omega)/\rho_n(\Omega)) \cdot \gamma_0$ we have, by property (B\ref{asp:ContinuityInterContinuity}),
\begin{align*}
C_K(\rho_n,\mnorm(\rho_n)) \leq J_K(\gamma_0,\gamma_1) = \int_{\Omega} c\big(x,1,x,\frac{\rho(\Omega)}{\rho_n(\Omega}\big) \d \rho_n(x) \to 0 \, .
\end{align*}
On the other hand, by choosing $\gamma_0 = \gamma_1$ equal to the optimal transport plan for the $W_{p,c}$ metric between $\rho$ and $\mnorm(\rho_n)$, we have by property (B\ref{asp:ContinuityInterEquivalence}),
\[
C_K(\mnorm(\rho_n),\rho)
 \leq \int_{\Omega^2} c(x,1,y,1) \d \gamma_0
 \to 0
\]
and we conclude thus that $C_K(\rho_n,\rho)  \to 0$.
\end{proof}
\fi

%%%%%%%%% DUALITY
Let us now give a dual formulation of the problem. It is similar to the dual formulation of the Kantorovich problem where one maximizes $\int \phi \d \rho_0 + \int \psi \d \rho_1$ over the set of pairs of continuous functions $(\phi,\psi)$ on $\Omega$ that satisfy $\phi(x)+\psi(y) \leq c(x,y)$. Here the objective is the same, but the constraint set is generally not a linear constraint set and is modified as follows.

\begin{definition}[Dual contraint set]\label{def:dualconstraint}
The dual constraint set $Q:\Omega^2 \to 2^{\R\times\R}$ is a set valued function defined, for all $(x,y)\in \Omega^2$ as the polar set to the function $c(x,\cdot,y\cdot)$, i.e.\ the domain of its convex conjugate.
\end{definition}

Remember that since the cost function $c$ is jointly 1-homogeneous, convex, and l.s.c.\ in the variables $(m_0,m_1)$, for all $(x,y)\in \Omega^2$, the Legendre transform of $c(x,\cdot,y,\cdot)$ is the indicator of a closed convex set. Moreover, as $c$ is nonnegative, and worth $+\infty$ if $m_0$ or $m_1$ is negative, the latter contains the negative orthant. We now state the dual problem (note that we do not attempt to prove the existence of dual maximizers).

%For nonempty convex valued multifunctions, $Q$ is said to be \emph{lower semicontinuous} if $G=\{(x,t) : x \in \tn{int } Q(t)\}$ is open (see \cite[Lemma 2]{rockafellar1971integrals}).

\begin{proposition}[Duality]
\label{prop: duality}
Let $c$ be a \emph{cost function}, $Q$ the associated dual constraint set from Definition~\ref{def:dualconstraint} and let
\[ 
B =  \left\{ (\phi, \psi) \in C(\Omega)^2 :  \forall (x,y) \in \Omega^2, (\phi(x),\psi(y)) \in Q(x,y) \right\}\,.
\]
Then
\[
C_K(\rho_0,\rho_1) =
 \sup_{(\phi, \psi) \in B} \int_{\Omega} \phi(x) \d \rho_0 + \int_{\Omega} \psi(y) \d \rho_1 
 %= \min_{(\gamma_0, \gamma_1)\in \Gamma(\rho_0, \rho_1)} J_K(\gamma_0, \gamma_1)  \, .
\]
\end{proposition}

\begin{corollary}[Sublinearity]\label{cor:sublinearityCK}
As the supremum of continuous linear functionals, $C_K$ is a sublinear (i.e.\ convex, positively $1$-homogeneous) and weakly* lower semicontinuous functional on $\mathcal{M}(\Omega)^2$.
\end{corollary}

\begin{proof}
Let us rewrite  the supremum problem as
\[
\sup_{(u_0,u_1) \in (C(\Omega^2)^2} - F(u_0,u_1) - G(u_0,u_1)
\]
where
\begin{align*}
G &: (u_0,u_1) \mapsto 
\begin{cases}
- \int_{\Omega}  \phi(x) \d \rho_0 -  \int_{\Omega} \psi(y) \d \rho_1  & \tn{if } u_0(x,y)=\phi(x) \\
		& \tn{and } u_1(x,y) = \psi(y) \\
+ \infty &\tn{otherwise,}
\end{cases} 
\end{align*}
and $F$ is the indicator of $\{ (u_0,u_1)\in (C(\Omega^2)^2) : (u_0,u_1)(x,y) \in Q(x,y), \, \forall (x,y)\in \Omega^2 \}$.
Note that $F$ and $G$ are convex and proper. Also, given our assumptions, there is a pair of functions $(u_0,u_1)$ at which $F$ is continuous (for the $\sup$ norm topology) and $F$ and $G$ are finite since for all $(x,y)\in \Omega^2$, $Q(x,y)$ contains the negative orthant. Then Fenchel-Rockafellar duality theorem (see, e.g.\ \cite[Theorem 1.9]{cedric2003topics}) states that
 \begin{equation}
 \label{eq: Fenchel-Rockafellar}
 \sup_{(u_0,u_1) \in C(\Omega^2)^2} \!\!\!\!\!\! - F(u_0,u_1) - G(u_0,u_1) 
 = 
 \!\!\!\!\!\!\min_{(\gamma_0, \gamma_1) \in \mathcal{M}(\Omega^2)^2} \!\!\!\!\! \left\{ F^*(\gamma_0,\gamma_1) + G^*(-\gamma_0,-\gamma_1) \right\} .
 \end{equation}
Let us compute the Legendre transforms. For $G$, we obtain
\begin{align*}
G^*(-\gamma_0,-\gamma_1) 
&= \!\!\!\!\!\! \sup_{(\phi,\psi)\in C(\Omega)^2} \!\!\!\! - \int_{\Omega^2} \phi(x)\d \gamma_0 - \int_{\Omega^2} \psi(x)\d \gamma_1 + \int_{\Omega} \phi(x) \d \rho_0 + \int_{\Omega} \psi(y) \d \rho_1\\
&= 
\begin{cases}
0 & \tn{ if } (\gamma_0, \gamma_1)\in \Gamma^{+/-}_{\rho_0, \rho_1}\\
+ \infty & \tn{ otherwise.}
\end{cases}
\end{align*}
where $\Gamma^{+/-}_{\rho_0, \rho_1} $ is the set of semi-couplings without the non-negativity constraint. On the other hand, by Lemma~\ref{lem:dualitymeasures},
\[
F^*(\gamma_0,\gamma_1) = 
\int_{\Omega^2} c\left(x, \dens{ \gamma_0}{ \gamma},y, \dens{ \gamma_1}{ \gamma} \right) \d\gamma(x,y) 
\]
where $\gamma$ is any measure in $\mathcal{M}_+(\Omega^2)$ with respect to which $(\gamma_0,\gamma_1)$ is absolutely continuous. %Note that this duality result requires $Q$ to be lower-semicontinuous in a sense which is equivalent to the lower-semicontinuity of $c$, thanks to \cite[Lemma A.2]{bouchitte1988integral}. 
Finally, as $F^*$ includes the nonnegativity constraint, the right hand side of \eqref{eq: Fenchel-Rockafellar} is equal to $\min_{(\gamma_0,\gamma_1)\in \Gamma(\rho_0,\rho_1)} J_K(\gamma_0,\gamma_1)$.
\end{proof}


%\todo{Mention $c$-conjugacy. we do not prove existence.}
%%%%%%%%%%%%
%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
% COMMENTED SECTION 
% COMMENTED SECTION 
%%%%%%%%%%%%%%%%%%%%%%%%%
% MonGE
%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\subsection{A formulation with deterministic semi-couplings}
By analogy with the Monge formulation of optimal transport, we can rewrite the problem in the particular case where the semi-couplings are generated by a map.
\begin{definition}[Monge-like Problem]
	For fixed marginals $\rho_0, \, \rho_1\in \mathcal{M}_+(\Omega)$, an auxiliary measure $\hat{\rho}_1 \in \mathcal{M}_+(\Omega)$ and a measurable map $T : \Omega \rightarrow \Omega$ satisfying $\pfwd{T} \hat{\rho}_1 = \rho_1$, it holds
\[
 \left( \pfwd{(\id,T)} \rho_0\, , \, \pfwd{(\id,T)} \hat{\rho}_1 \right) \in \Gamma(\rho_0,\rho_1)\, .
\]
We define a Monge-like functional by
	\begin{align*}
		J_M(\rho_0,\hat{\rho}_1,T) & = J_K \left( \vphantom{\sum}
			\pfwd{(\id,T)} \rho_0,
			\pfwd{(\id,T)} \hat{\rho}_1
			\right) \\
			& = \int_{\Omega} c\big(x,T(x),\rho_0(x),\hat{\rho}_1(x)\big)\,dx
	\end{align*}
	and the corresponding optimization problem as
	\[
		C_M(\rho_0,\rho_1) = \inf_{\hat{\rho}_1 , T}
			J_M(\rho_0,\hat{\rho}_1,T)
			\qquad  \tn{subject to}\qquad \pfwd{T} \hat{\rho}_1 = \rho_1\, .
	\]
with the convention that this infimum is $+\infty$ when the feasible set is empty.
\end{definition}
\begin{proposition}
\label{th : inequality monge static}
For $\rho_0,\, \rho_1 \in \mathcal{M}_+(\Omega)$, we have $C_K(\rho_0,\rho_1) \leq C_M(\rho_0,\rho_1)$.
\end{proposition}

\begin{proof}
It is direct since $C_M$ is obtained by minimizing $J_K$ over a subset of $\Gamma(\rho_0, \rho_1)$.
\end{proof}
\fi



